Classification with Strategically Withheld Data

Machine learning techniques can be useful in applications such as credit approval and college admission. However, to be classified more favorably in such contexts, an agent may decide to strategically withhold some of her features, such as bad test scores. This is a missing data problem with a twist: which data is missing {\em depends on the chosen classifier}, because the specific classifier is what may create the incentive to withhold certain feature values. We address the problem of training classifiers that are robust to this behavior. We design three classification methods: {\sc Mincut}, {\sc Hill-Climbing} ({\sc HC}) and Incentive-Compatible Logistic Regression ({\sc IC-LR}). We show that {\sc Mincut} is optimal when the true distribution of data is fully known. However, it can produce complex decision boundaries, and hence be prone to overfitting in some cases. Based on a characterization of truthful classifiers (i.e., those that give no incentive to strategically hide features), we devise a simpler alternative called {\sc HC} which consists of a hierarchical ensemble of out-of-the-box classifiers, trained using a specialized hill-climbing procedure which we show to be convergent. For several reasons, {\sc Mincut} and {\sc HC} are not effective in utilizing a large number of complementarily informative features. To this end, we present {\sc IC-LR}, a modification of Logistic Regression that removes the incentive to strategically drop features. We also show that our algorithms perform well in experiments on real-world data sets, and present insights into their relative performance in different settings.

==> notes.tex <==
\section{Notes}
\anilesh{
\begin{itemize}
    \item why is the error bar higher for some in Fig 1? Look at a bunch of single runs?
    \item tough to run monotonic with a lot of binary / plain categorical? for each dataset, check which of the categorical variables are ordered, and if there are at least a few, we can try monotonic mincut also.
    \item try AUC for the second fig and see how it looks? \hl{done}
    \item add a few continuous features and see what happens to mincut?
    \item generalization: can we regularize the meta-classifier?
    \item can we do anything with more features where strategic behavior happens?
    \item voting ensembles? \hl{future work}
    \item order of training the classifier within greedy.
    \item majority nearest neighbor
    \item top 4 numerical features -- or different types of features 
    \item why is NN not doing well? Don't claim that they cannot do well ever?
    \item other methods on all features -- otherwise handicapping those methods \hl{cannot test strategic behavior -- too many combinations}
    \item are the lower ones accepting everything
    \item 5/5: 1. N.Neigh non-strategic 2. monotonic
    \item make sure we are not inventing new methods 
    \item still do basic nearest neighbors!
    (KNN)
\end{itemize}}

==> prelims_old.tex <==
\section{Preliminaries}
\label{sec:prelim}

In this section, we briefly review the PAC learning model under which we will develop our theoretical results, and discuss how strategically dropped features fit in the classical model.

\paragraph{The PAC learning model.}
In the classical PAC learning model, there is a feature space $\mathcal{X}$, a label space $\mathcal{Y} = \{0, 1\}$, and a distribution $\mathcal{D}$ over $\mathcal{X} \times \mathcal{Y}$ which models the population.
A classifier $f: \mathcal{X} \to \mathcal{Y}$ maps a combination of features to a label.
The (population) {\em loss} of a truthful classifier $f$ is defined to be
\[
    \ell_\mathcal{D}(f) = \Pr_{(x, y) \sim \mathcal{D}}[f(x) \ne y].
\]
The smaller the loss is, the better quality the classifier is of.
The goal of PAC learning is to compute a classifier of as small loss as possible, given access to iid labelled samples from the population distribution $\mathcal{D}$.
Note that how small the loss can be generally depends on the number of samples observed.

\paragraph{Strategically dropped features.}
We now extend the PAC learning model to the setting we consider, where features can be strategically dropped.
Let $F = [k] = \{1, \dots, k\}$ be the set of features, each of which a data point may or may not have.
For a data point $x \in \mathcal{X}$, let $x_i$ denote the value of its $i$-th feature.
$x_i = *$ if $x$ does not have feature $i \in [k]$.
For any set of features $S \subseteq [k]$, let $x|_S$ be $x$ projected to $S$, obtained by dropping all features out of $S$.
That is,
\[
    (x|_S)_i =
    \begin{cases}
        x_i, & \text{if } i \in S \\
        *, & \text{otherwise}.
    \end{cases}
\]
A data point with feature values $x$ can report feature values $x'$ (denoted $x \to x'$), iff there exists a set of features $S \subseteq [k]$, such that $x|_S = x'$.
$S = [k]$ corresponds to the case where a data point can always report its complete feature values.
Note that $\to$ is transitive, i.e., for any $x_1, x_2, x_3 \in \mathcal{X}$,
\[
    x_1 \to x_2 \text{ and } x_2 \to x_3 \Longrightarrow x_1 \to x_3.
\]
We assume data points prefer label $1$ to $0$.
In response to a classifier $f$, a data point with feature values $x$ will always drop (or not drop) features in a way such that they receive label $1$ whenever possible, i.e., it will report
\[
    x' \in \argmax_{x'': x \to x''} f(x'').
\]
Such strategic behavior in general affects the loss of the classifier.
Formally, with strategically dropped features, the loss of a classifier $f$ is
\[
    \ell_\mathcal{D}(f) = \Pr_{(x, y) \sim \mathcal{D}}\left[\max_{x': x \to x'} f(x') \ne y\right].
\]

\paragraph{Truthful classifiers.}
Strategically dropped features can be undesirable in various ways.
One may therefore be interested in {\em truthful} classifiers, which provably prevent such strategic manipulation.
A classifier $f$ is truthful, if for any $x, x' \in \mathcal{X}$ where $x \to x'$, $f(x) \ge f(x')$.
In other words, reporting ones complete feature values is always an optimal way to respond to a truthful classifier.
As a result, the loss of any truthful classifier $f$ in the presence of strategically dropped features has the same form of the loss in the classical PAC model, i.e.,
\[
    \ell_\mathcal{D}(f) = \Pr_{(x, y) \sim \mathcal{D}}[f(x) \ne y].
\]
Note that since the reporting structure is transitive, the so-called revelation principal holds (see \cite{zhang2019distinguishing}), which states that any classifier $f$ is equivalent to a truthful classifier $f'$.
Formally, for any classifier $f$, there exists a truthful classifier $f'$, such that for any $x \in \mathcal{X}$,
\[
    \max_{x': x \to x'} f(x') = f'(x).
\]
So without loss of generality, one can focus on truthful classifiers.

==> references.tex <==
\begin{thebibliography}{40}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Adams(2017)]{adams2017race}
Caralee~J. Adams.
\newblock \emph{In Race for Test-Takers, ACT Outscores SAT—for Now}, 2017.
\newblock URL
  \url{https://www.edweek.org/ew/articles/2017/05/24/in-race-for-test-takers-act-outscores-sat--for.html}.

\bibitem[Amodei et~al.(2016)Amodei, Olah, Steinhardt, Christiano, Schulman, and
  Man{\'e}]{Amodei2016ConcretePI}
Dario Amodei, Chris Olah, Jacob Steinhardt, Paul~F. Christiano, John Schulman,
  and Dan Man{\'e}.
\newblock Concrete problems in ai safety.
\newblock \emph{ArXiv}, abs/1606.06565, 2016.

\bibitem[Chawla et~al.(2003)Chawla, Japkowicz, and Kolcz]{chawla2003icml}
N~Chawla, N~Japkowicz, and A~Kolcz.
\newblock Icml’2003 workshop on learning from imbalanced data sets (ii).
\newblock In \emph{Proceedings available at http://www. site. uottawa.
  ca/nat/Workshop2003/workshop2003. html}, 2003.

\bibitem[Chawla et~al.(2004)Chawla, Japkowicz, and Kotcz]{chawla2004special}
Nitesh~V Chawla, Nathalie Japkowicz, and Aleksander Kotcz.
\newblock Special issue on learning from imbalanced data sets.
\newblock \emph{ACM SIGKDD explorations newsletter}, 6\penalty0 (1):\penalty0
  1--6, 2004.

\bibitem[Chen et~al.(2018)Chen, Podimata, Procaccia, and
  Shah]{chen2018strategyproof}
Yiling Chen, Chara Podimata, Ariel~D Procaccia, and Nisarg Shah.
\newblock Strategyproof linear regression in high dimensions.
\newblock In \emph{Proceedings of the 2018 ACM Conference on Economics and
  Computation}, pages 9--26, 2018.

\bibitem[Conroy et~al.(2016)Conroy, Eshelman, Potes, and
  Xu-Wilson]{conroy2016dynamic}
Bryan Conroy, Larry Eshelman, Cristhian Potes, and Minnan Xu-Wilson.
\newblock A dynamic ensemble approach to robust classification in the presence
  of missing data.
\newblock \emph{Machine Learning}, 102\penalty0 (3):\penalty0 443--463, 2016.

\bibitem[Cormen et~al.(2009)Cormen, Leiserson, Rivest, and
  Stein]{cormen2009introduction}
Thomas~H Cormen, Charles~E Leiserson, Ronald~L Rivest, and Clifford Stein.
\newblock \emph{Introduction to algorithms}.
\newblock MIT press, 2009.

\bibitem[Dalvi et~al.(2004)Dalvi, Domingos, Sanghai, and
  Verma]{dalvi2004adversarial}
Nilesh Dalvi, Pedro Domingos, Sumit Sanghai, and Deepak Verma.
\newblock Adversarial classification.
\newblock In \emph{Proceedings of the tenth ACM SIGKDD international conference
  on Knowledge discovery and data mining}, pages 99--108, 2004.

\bibitem[Daniely et~al.(2015)Daniely, Sabato, Ben-David, and
  Shalev-Shwartz]{daniely2015multiclass}
Amit Daniely, Sivan Sabato, Shai Ben-David, and Shai Shalev-Shwartz.
\newblock Multiclass learnability and the erm principle.
\newblock \emph{The Journal of Machine Learning Research}, 16\penalty0
  (1):\penalty0 2377--2404, 2015.

\bibitem[Dekel et~al.(2010{\natexlab{a}})Dekel, Fischer, and
  Procaccia]{dekel2010incentive}
Ofer Dekel, Felix Fischer, and Ariel~D Procaccia.
\newblock Incentive compatible regression learning.
\newblock \emph{Journal of Computer and System Sciences}, 76\penalty0
  (8):\penalty0 759--777, 2010{\natexlab{a}}.

\bibitem[Dekel et~al.(2010{\natexlab{b}})Dekel, Shamir, and
  Xiao]{dekel2010learning}
Ofer Dekel, Ohad Shamir, and Lin Xiao.
\newblock Learning to classify with missing and corrupted features.
\newblock \emph{Machine learning}, 81\penalty0 (2):\penalty0 149--178,
  2010{\natexlab{b}}.

\bibitem[Dietterich(1998)]{dietterich1998approximate}
Thomas~G Dietterich.
\newblock Approximate statistical tests for comparing supervised classification
  learning algorithms.
\newblock \emph{Neural computation}, 10\penalty0 (7):\penalty0 1895--1923,
  1998.

\bibitem[Dua and Graff(2017)]{Dua:2019}
Dheeru Dua and Casey Graff.
\newblock {UCI} machine learning repository, 2017.
\newblock URL \url{http://archive.ics.uci.edu/ml}.

\bibitem[Elkan(2001)]{elkan2001foundations}
Charles Elkan.
\newblock The foundations of cost-sensitive learning.
\newblock In \emph{International joint conference on artificial intelligence},
  volume~17, pages 973--978. Lawrence Erlbaum Associates Ltd, 2001.

\bibitem[Fayyad and Irani(1993)]{DBLP:conf/ijcai/FayyadI93}
Usama~M. Fayyad and Keki~B. Irani.
\newblock Multi-interval discretization of continuous-valued attributes for
  classification learning.
\newblock In Ruzena Bajcsy, editor, \emph{Proceedings of the 13th International
  Joint Conference on Artificial Intelligence. Chamb{\'{e}}ry, France, August
  28 - September 3, 1993}, pages 1022--1029. Morgan Kaufmann, 1993.
\newblock URL \url{http://ijcai.org/Proceedings/93-2/Papers/022.pdf}.

\bibitem[Florez-Lopez(2010)]{florezlopez2010effects}
Raquel Florez-Lopez.
\newblock Effects of missing data in credit risk scoring. a comparative
  analysis of methods to achieve robustness in the absence of sufficient data.
\newblock \emph{The Journal of the Operational Research Society}, 61\penalty0
  (3):\penalty0 486--501, 2010.

\bibitem[Globerson and Roweis(2006)]{globerson2006nightmare}
Amir Globerson and Sam Roweis.
\newblock Nightmare at test time: robust learning by feature deletion.
\newblock In \emph{Proceedings of the 23rd international conference on Machine
  learning}, pages 353--360, 2006.

\bibitem[Green and Laffont(1986)]{green1986partially}
Jerry~R Green and Jean-Jacques Laffont.
\newblock Partially verifiable information and mechanism design.
\newblock \emph{The Review of Economic Studies}, 53\penalty0 (3):\penalty0
  447--456, 1986.

\bibitem[Haghtalab et~al.(2020)Haghtalab, Immorlica, Lucier, and
  Wang]{haghtalab2020maximizing}
Nika Haghtalab, Nicole Immorlica, Brendan Lucier, and Jack Wang.
\newblock Maximizing welfare with incentive-aware evaluation mechanisms.
\newblock In \emph{29th International Joint Conference on Artificial
  Intelligence}, 2020.

\bibitem[Hand and Anagnostopoulos(2013)]{hand2013area}
David~J Hand and Christoforos Anagnostopoulos.
\newblock When is the area under the receiver operating characteristic curve an
  appropriate measure of classifier performance?
\newblock \emph{Pattern Recognition Letters}, 34\penalty0 (5):\penalty0
  492--495, 2013.

\bibitem[Hardt et~al.(2016)Hardt, Megiddo, Papadimitriou, and
  Wootters]{hardt2016strategic}
Moritz Hardt, Nimrod Megiddo, Christos Papadimitriou, and Mary Wootters.
\newblock Strategic classification.
\newblock In \emph{Proceedings of the 2016 ACM conference on innovations in
  theoretical computer science}, pages 111--122, 2016.

\bibitem[Japkowicz(2000)]{japkowicz2000aaai}
N~Japkowicz.
\newblock Aaai’2000 workshop on learning from imbalanced data sets.
\newblock \emph{AAAI Tech Report, No. WS-00-05}, 2000.

\bibitem[Jung et~al.(2017)Jung, Concannon, Shroff, Goel, and
  Goldstein]{jung2017simple}
Jongbin Jung, Connor Concannon, Ravi Shroff, Sharad Goel, and Daniel~G
  Goldstein.
\newblock Simple rules for complex decisions.
\newblock \emph{Available at SSRN 2919024}, 2017.

\bibitem[Kephart and Conitzer(2015)]{kephart2015complexity}
Andrew Kephart and Vincent Conitzer.
\newblock Complexity of mechanism design with signaling costs.
\newblock In \emph{Proceedings of the 2015 International Conference on
  Autonomous Agents and Multiagent Systems}, pages 357--365, 2015.

\bibitem[Kephart and Conitzer(2016)]{kephart2016revelation}
Andrew Kephart and Vincent Conitzer.
\newblock The revelation principle for mechanism design with reporting costs.
\newblock In \emph{Proceedings of the 2016 ACM Conference on Economics and
  Computation}, pages 85--102, 2016.

\bibitem[Kleinberg and Raghavan(2019)]{kleinberg2019classifiers}
Jon Kleinberg and Manish Raghavan.
\newblock How do classifiers induce agents to invest effort strategically?
\newblock In \emph{Proceedings of the 2019 ACM Conference on Economics and
  Computation}, pages 825--844, 2019.

\bibitem[Lessmann et~al.(2015)Lessmann, Baesens, Seow, and
  Thomas]{lessmann2015benchmarking}
Stefan Lessmann, Bart Baesens, Hsin-Vonn Seow, and Lyn~C Thomas.
\newblock Benchmarking state-of-the-art classification algorithms for credit
  scoring: An update of research.
\newblock \emph{European Journal of Operational Research}, 247\penalty0
  (1):\penalty0 124--136, 2015.

\bibitem[Marlin(2008)]{marlin2008missing}
Benjamin Marlin.
\newblock \emph{Missing data problems in machine learning}.
\newblock PhD thesis, Citeseer, 2008.

\bibitem[Pedregosa et~al.(2011)Pedregosa, Varoquaux, Gramfort, Michel, Thirion,
  Grisel, Blondel, Prettenhofer, Weiss, Dubourg, Vanderplas, Passos,
  Cournapeau, Brucher, Perrot, and Duchesnay]{scikit-learn}
F.~Pedregosa, G.~Varoquaux, A.~Gramfort, V.~Michel, B.~Thirion, O.~Grisel,
  M.~Blondel, P.~Prettenhofer, R.~Weiss, V.~Dubourg, J.~Vanderplas, A.~Passos,
  D.~Cournapeau, M.~Brucher, M.~Perrot, and E.~Duchesnay.
\newblock Scikit-learn: Machine learning in {P}ython.
\newblock \emph{Journal of Machine Learning Research}, 12:\penalty0 2825--2830,
  2011.

\bibitem[Saar-Tsechansky and Provost(2007)]{saar2007handling}
Maytal Saar-Tsechansky and Foster Provost.
\newblock Handling missing values when applying classification models.
\newblock \emph{Journal of machine learning research}, 8\penalty0
  (Jul):\penalty0 1623--1657, 2007.

\bibitem[Shalev-Shwartz and Ben-David(2014)]{shalev2014understanding}
Shai Shalev-Shwartz and Shai Ben-David.
\newblock \emph{Understanding machine learning: From theory to algorithms}.
\newblock Cambridge university press, 2014.

\bibitem[Syed and Taskar(2010)]{syed2010semi}
Umar Syed and Ben Taskar.
\newblock Semi-supervised learning with adversarially missing label
  information.
\newblock In \emph{Advances in Neural Information Processing Systems}, pages
  2244--2252, 2010.

\bibitem[Vorobeychik and Kantarcioglu(2018)]{vorobeychik2018adversarial}
Yevgeniy Vorobeychik and Murat Kantarcioglu.
\newblock Adversarial machine learning.
\newblock \emph{Synthesis Lectures on Artificial Intelligence and Machine
  Learning}, 12\penalty0 (3), 2018.

\bibitem[Wang and Rudin(2015)]{wang2015falling}
Fulton Wang and Cynthia Rudin.
\newblock Falling rule lists.
\newblock In \emph{Artificial Intelligence and Statistics}, pages 1013--1022,
  2015.

\bibitem[Yu(2011)]{yu2011mechanism}
Lan Yu.
\newblock Mechanism design with partial verification and revelation principle.
\newblock \emph{Autonomous Agents and Multi-Agent Systems}, 22\penalty0
  (1):\penalty0 217--223, 2011.

\bibitem[Zhang and Conitzer(2021)]{zhang2021incentive}
Hanrui Zhang and Vincent Conitzer.
\newblock Incentive-aware {PAC} learning.
\newblock In \emph{Proceedings of the AAAI Conference on Artificial
  Intelligence}, 2021.

\bibitem[Zhang et~al.(2019{\natexlab{a}})Zhang, Cheng, and
  Conitzer]{zhang2019distinguishing}
Hanrui Zhang, Yu~Cheng, and Vincent Conitzer.
\newblock Distinguishing distributions when samples are strategically
  transformed.
\newblock In \emph{Advances in Neural Information Processing Systems}, pages
  3187--3195, 2019{\natexlab{a}}.

\bibitem[Zhang et~al.(2019{\natexlab{b}})Zhang, Cheng, and
  Conitzer]{zhang2019samples}
Hanrui Zhang, Yu~Cheng, and Vincent Conitzer.
\newblock When samples are strategically selected.
\newblock In \emph{International Conference on Machine Learning}, pages
  7345--7353, 2019{\natexlab{b}}.

\bibitem[Zhang et~al.(2021{\natexlab{a}})Zhang, Cheng, and
  Conitzer]{zhang2021automated}
Hanrui Zhang, Yu~Cheng, and Vincent Conitzer.
\newblock Automated mechanism design for classification with partial
  verification.
\newblock In \emph{Proceedings of the AAAI Conference on Artificial
  Intelligence}, 2021{\natexlab{a}}.

\bibitem[Zhang et~al.(2021{\natexlab{b}})Zhang, Cheng, and
  Conitzer]{zhang2021classification}
Hanrui Zhang, Yu~Cheng, and Vincent Conitzer.
\newblock Classification with few tests through self-selection.
\newblock In \emph{Proceedings of the AAAI Conference on Artificial
  Intelligence}, 2021{\natexlab{b}}.

\end{thebibliography}


==> strategic classification arxiv/abstract.tex <==
%\vc{Did we try to reorder the beginning? I'm OK either way.}
%Classification in the presence of missing data is a common problem in machine learning. This problem can be compounded when making decisions about strategic agents in settings such as credit approval, college admissions, etc. To the extent that we rely on agents to submit data about themselves, they may strategically hide some of their features in order to be classified more favorably. In this paper, we address the problem of training classifiers that are robust to this behavior.

Machine learning techniques can be useful in applications such as credit approval and college admission. However, to be classified more favorably in such contexts, an agent may decide to strategically withhold some of her features, such as bad test scores.  This is a missing data problem with a twist: which data is missing {\em depends on the chosen classifier}, because the specific classifier is what may create the incentive to withhold certain feature values. We address the problem of training classifiers that are robust to this behavior.

We design three classification methods: {\sc Mincut}, {\sc Hill-Climbing} ({\sc HC}) and Incentive-Compatible Logistic Regression ({\sc IC-LR}). We show that {\sc Mincut} is optimal when the true distribution of data is fully known. However, it can produce complex decision boundaries, and hence be prone to overfitting in some cases. Based on a characterization of truthful classifiers (i.e., those that give no incentive to strategically hide features), we devise a simpler alternative called {\sc HC} which consists of a hierarchical ensemble of out-of-the-box classifiers, trained using a specialized hill-climbing procedure which we show to be convergent. For several reasons, {\sc Mincut} and {\sc HC} are not effective in utilizing a large number of complementarily informative features. To this end, we present {\sc IC-LR}, a modification of Logistic Regression that removes the incentive to strategically drop features. We also show that our algorithms perform well in experiments on real-world data sets, and present insights into their relative performance in different settings.

%\david{Some classification problems involve strategic agents, such as determining whether to grant someone a loan, admission to university, etc. To the extent that we rely on agents to submit data about themselves, they may strategically hide some of their features in order to be classified more favorably. If there is data missing for non-strategic reasons, which occurs often in machine learning, classification becomes difficult. In this paper, we address the problem of training classifiers that are robust to this behavior.}

%, such as determining whether to grant someone a loan, admission, etc. \hl{(... e.g. 
%can handle strategically missing data at prediction time (i.e., assuming we have a truthfully reported test set with naturally missing data).

%\hl{Classification aids the principal to make decisions about agents in applications such as credit approval and college admission. However, to be classified more favorably, an agent can complicate the problem by strategically withholding some of her features. This problem becomes nontrivial to the principal in the presence of other agents' non-strategic, naturally missing features, common in machine learning. In this paper, ... (Same order of reasoning as David's, but different use of words and phrases and hopefully reads better)}

%\hl{Classification aids decision-making in applications such as credit approval and college admission. However, to be classified more favorably, an agent can complicate the problem by strategically withholding some of her features. This problem becomes nontrivial to in the presence of other agents' non-strategic, naturally missing features, common in machine learning. In this paper, ... (... if we don't want to mention principal-agent, although IMO we should)}

%\hl{(... that guarantees to converge (I personally prefer "an algorithm converges" to "an algorithm is convergent"))}. \david{how about: ''which we show converges"? }\anilesh{I think ``to be convergent" is better grammatically.} \hl{Google "algorithm converges" returns 500k result whereas "algorithm is convergent" returns 100k, but your call}

==> strategic classification arxiv/broader_impact.tex <==
\section*{Acknowledgements}

We are thankful for support from NSF under award IIS-1814056.

\section*{Ethics Statement}

The methods presented in this paper are geared towards preventing the strategic withholding of data when machine learning methods are used in real-world applications. This will increase the robustness of ML techniques in these contexts: without taking this issue into account, deployment of these techniques will generally result in a rapid change in the distribution of submitted data due to the new incentives faced, causing techniques to work much more poorly than expected at training time. Thus, there is an AI safety \citep{Amodei2016ConcretePI} benefit to our work. The lack of strategic withholding also enables the collection of (truthful) quality data. Of course, there can be a downside to this as well if the data is not used responsibly, which could be the case especially if the features that (without our techniques) would have been withheld are sensitive or private in nature. 

The other issues to consider in our context are those of transparency and fairness. We assume that the classifier is public knowledge, and therefore, agents can appropriately best-respond. In practice, this might not be the case; however, agents may learn how to best-respond over time if similar decisions are made repeatedly (e.g., in the case of college admissions or loan applications). While US college admission is often a black box, it need not be; many countries have transparent public criteria for university admissions (e.g., the Indian IIT admission system), and the same is true in many other contexts (e.g., Canadian immigration). Of course, transparency goes hand in hand with interpretability, i.e., the classifier must be easily explainable as well, and there could be a trade-off, in principle, between how easy the classifier is to interpret and the accuracy it can achieve. It is also possible that our methods hurt the chances of those with more missing data (similarly to how immigrants without credit history may not be able to get a credit card). This is to some extent inevitable, because if one can get in without any feature, everyone could get in by dropping all features. Therefore, the issue of fairness might arise in the case where some groups systematically tend to have more missing data.

==> strategic classification arxiv/conclusion.tex <==
\section{Conclusion}
% In this paper, we studied the problem of classification when each agent at prediction time can strategically withhold some of its features to obtain a more favorable outcome. We devised classification methods that are robust to this behavior. We presented the {\sc Mincut} classifier, which is optimal given full knowledge of the input distribution. We characterized the space of all possible truthful classifiers in our setting, as well as the {\sc Hill-Climbing} and the Incentive-Compatible Logistic Regression methods. We tested these methods on real-world data sets, showing \begin{enumerate*}[label = (\alph*)]
%     \item how they perform in different settings, and 
%     \item that they outperform out-of-the-box methods that do not account for the aforementioned strategic behavior.
% \end{enumerate*}

In this paper, we studied the problem of classification when each agent at prediction time can strategically withhold some of its features to obtain a more favorable outcome. We devised classification methods ({\sc Mincut}, {\sc HC} and {\sc IC-LR}) that are robust to this behavior, and in addition, characterized the space of all possible truthful classifiers in our setting. We tested our methods on real-world data sets, showing that they outperform out-of-the-box methods that do not account for the aforementioned strategic behavior. 

%There is rich literature on dealing with missing data in general \citep{rubin1976inference,batista2003analysis,saar2007handling}. We complement this line of research by focusing on the specific case where data is missing for strategic reasons. 

%In order to train a classifier using the {\sc HC} methodology, we start by selecting a small number of features from the data. This comes at little cost on the data sets that we test on -- most of the information useful for prediction is contained within these features. Therefore, most standard methods perform very similarly whether they are applied to all the features or just these. And it is natural to expect that using a smaller number of features diminishes the damage done by strategic behavior under most reasonable classifiers. The other reason is that having a small number of features makes it easy to train {\sc Mincut} and {\sc HC}.
%Still, an interesting open question is to extend these techniques to settings in which it is important to use a large number of features.
%An interesting open question is to figure out how to compare methods that account for strategic behavior and those that do not, on a large set of features. 
%One plausible avenue for tractable truthful methods in higher dimensions could be the use of voting based methods.\vc{references?  but I think this is too vague as written here; I don't think someone reading this quickly will have any idea what the point is.  We could expand, but then it just invites the criticism that we should have tested that too, instead of just making an unsupported claim in the paper that this is likely to work well.  I'm inclined to leave it out (of course maybe we won't have space for the whole paragraph / conclusion anyway...)}

 An immediate question that follows is relaxing the assumption of having access to truthful training data -- for example, one could ask what the best incentive-compatible classifier is given that the training data consists of best responses to a known classifier $f$; or, one could consider an online learning model where the goal is to bound the overall loss over time. A much broader question for future work is to develop a more general theory of robustness to missing data that naturally includes the case of strategic withholding.
%\vc{changed this last sentence because what it said before suggested that we were not ``harmonious'' with these other methods, which I think is also not true...}
%Another interesting question is to see if these two potential sources of missing data can be dealt with together in a harmonious fashion. How best to do so is a question we leave for future work.
\newpage

==> strategic classification arxiv/experiments.tex <==
\section{Evaluation} \label{sec:experiments}

In this section, we show that, when strategic withholding is at play, {\sc Mincut}, {\sc HC} and {\sc IC-LR} perform well and provide a significant advantage over several out-of-the-box counterparts (that do not account for strategic behavior).  
\paragraph{Datasets} Four credit approval datasets are obtained from the UCI repository \citep{Dua:2019}, one each from Australia, Germany, Poland and Taiwan. As is common for credit approval datasets, they are imbalanced to various degrees. In order to demonstrate the performance of classifiers in a standard, controlled setting, we balance them by random undersampling. There is a dedicated community \citep{chawla2004special} that looks at the issue of imbalanced learning. We do not delve into these issues in our paper, and evaluate our methods on both balanced and imbalanced datasets (see the Supplement for the latter). In addition, to demonstrate the challenge of high-dimensional data imposed on some of the classification methods, the experiments are run on the datasets  
\begin{enumerate*}[label=(\alph*)]
    \item restricted to 4 features,\footnote{\scriptsize According to ANOVA F-value evaluated before dropping any feature values.} and 
    \item with all available features.
\end{enumerate*} 
The basic characteristics of the datasets are summarized in Table \ref{tab:summary} -- note that there is enough variation in terms of the types of features present.
We then randomly remove a fraction $\epsilon = 0, 0.1, \dots, 0.5$ of all feature values in each dataset to simulate data that is missing ``naturally'' -- i.e., not due to strategic withholding. 
\begin{table}
\centering
% \ra{1.3}
\small
\caption{Data set summary statistics (num. = numerical, cat. = categorical)}
\begin{tabular}{lcccc}\toprule
Data set & Size & \makecell{Total \# of \\ features} &  \makecell{Size after \\ balancing}  & \makecell{Features after\\ restriction}\\ \midrule
Australia & 690 & 15 & 614  & 2 num., 2 cat. \\
Germany & 1000 & 20 & 600 & 1 num., 3 cat. \\
Poland & 5910 & 64 & 820  & 4 num. \\
Taiwan & 30,000 & 23 & 13,272  & 4 ordinal \\
\bottomrule
\end{tabular}
\label{tab:summary}
\end{table}

\paragraph{Testing} We test all methods under two ways of reporting: ``truthful'', i.e., all features are reported as is, and ``strategic'', i.e., some features might be withheld if it leads to a better outcome. We measure the test accuracy of each classifier, averaged over N=100 runs, with randomness over the undersampling and the data that is randomly chosen to be missing, to simulate data missing for non-strategic reasons. Other metrics, and details about implementing and training the classifiers, are discussed in the Supplement. It is important to note that for testing any method, we have to, in effect, compute the best response of each data point toward the classifier. Since the methods we propose are truthful, this is a trivial task. But for other methods, this might not be easy, thereby limiting what baselines can be used. 



% We evaluate classifiers on the German and Australian credit dataset, two well-studied benchmark classification dataset
% \citep{baesens2003benchmarking}

% We believe that credit approval can be an application of our framework, as...
% \anilesh{Are there any other applications?} We randomly remove a fraction of the feature values in the dataset, to simulate the values missing by nature.

% For each data set, we use f-test to select the best subset of 5 features, as testing strategic behavior with more features becomes computationally intractable. We chose a univariate feature selection method as it does not favor any particular classifier in the testing stage (c.t. a model based feature selection method)


% \item We use t-test to select the best subset of 5 features. \cite{tsai2009feature} demonstrates that t-test is the best feature selection method on the two and the other benchmark credit scoring datasets, as it selects more representative variables to increase the performance of prediction.
% \anilesh{How would it work with post-deletion ground truth?}


\paragraph{Classifiers} We evaluate our proposed methods, {\sc Mincut}, {\sc HC} with logistic regression ({\sc HC (LR)}) and neural networks ({\sc HC (ANN)}) as subclassifiers, and incentive-compatible logistic regression (IC-LR), against several baseline methods.

First, they will be compared against three out-of-the-box baseline classifiers: logistic regression ({\sc LR}), neural networks ({\sc ANN}) and random forest ({\sc RF}). We select {\sc LR} for its popularity in credit approval applications; we select {\sc ANN} for it being the best-performing individual classifier on some credit approval datasets \citep{lessmann2015benchmarking}; we select RF for it being the best-performing homogeneous ensemble on some credit approval datasets \citep{lessmann2015benchmarking}, as {\sc HC} can be viewed as a homogeneous ensemble method. For the sake of exposition, we present numbers just for baselines based on LR, as they perform relatively better. %\anilesh{just LR because it performs better, and not enough space to have all these. Can include a couple more, but not sure that helps}
%\vc{but in the tables below there's only LR right (due to the others making it too hard to simulate strategic reporting?  though is this true with few features?) Should be careful not to confuse the reader even if things are in the appendix, which they likely won't read.  And we do still have some more space?}

Second, for the purposes of comparison, we include {\sc Maj} -- predict the \emph{majority} label if examples with the exact same feature values appeared in the training set, and reject if not -- which can be thought of as a non-strategic counterpart of {\sc Mincut}. We also include k-nearest neighbors ({\sc kNN}) as a baseline, since it is closely related to {\sc Maj}.

These out-of-the-box classifiers need help dealing with missing data, whether they are missing naturally at training and test time or strategically at test time, and to this end, we employ 
\begin{enumerate*}[label = (\alph*)]
    \item {\sc Imp}: mean/mode imputation \citep{lessmann2015benchmarking}, and
    \item {\sc R-F}: reduced-feature modeling \citep{saar2007handling},
\end{enumerate*}  
for each of them.

When the dataset has a large number of features, {\sc Mincut} and {\sc IC-LR} can be directly applied. For {\sc HC}, we assist it in two ways: \begin{enumerate*}[label=(\alph*)]
    \item by selecting 4 features based on the training data, denoted by {\sc fs} (feature selection),\footnote{\scriptsize Such a technique can be applied to other methods too -- the results (see the Supplement) are not very different from those in Tables \ref{tab:accuracy,_2_bal,AAAI,FS,disc}.} and
    \item by choosing a limited number of small subsets (30 with 1 feature and 30 with 2 features), denoted by {\sc app} (approximation).
\end{enumerate*} Note that since our proposed methods are truthful, we can assume that features are reported as is. However, for all out-of-the-box classifiers, except {\sc Imp(LR)}, it is infeasible to simulate strategic withholding of feature values, due to the enormous number of combinations of features.

Last but not least, we test all methods with the discretization of continuous features (into categorical ones) \citep{DBLP:conf/ijcai/FayyadI93}, for reasons given in earlier sections.

%, in strategic and non-strategic settings. 
% We select LR for its popularity in credit scoring and ANN for being the best-performing individual classifier on credit approval datasets \citep{lessmann2015benchmarking}.

% For the purposes of comparison, we include {\sc Maj} -- predict the \emph{majority} label if examples with the exact same feature values appeared in the training set, and reject if not -- which can be thought of as a non-strategic counterpart of {\sc Mincut}. We also include standard methods like kNN (k-Nearest Neighbors, which is intuitively similar to {\sc Maj}), and others such as ANN and LR. Since {\sc HC} is an ensemble method, RF (Random Forest), the best-performing homogeneous ensemble on credit approval datasets \citep{lessmann2015benchmarking}, is added to the mix. We use these out-of-the-box methods (kNN, LR, ANN, RF) by employing either mean/mode imputation \citep{lessmann2015benchmarking} or reduced-feature modeling \citep{saar2007handling}, to deal with missing data. We use {\sc Mincut}, {\sc HC}, and {\sc Maj} with and without discretization \citep{fayyad1992handling}. For the sake of our exposition here, we do not use discretization for Imputation and Reduced Feature methods, as it does not really help (see \textbf{Results} below, and also the Supplement).

% We will discretize the datasets because we assume that the data points define the distribution. Otherwise, mis-reporting to ... This is similar to how continuous features need to be discretized to generate a decision tree \citep{fayyad1992handling}. 

% \item We compare the performance of our greedy algorithm and min-cut solution against that of neural network (NN), logistic regression (LR) and random forest (RF). We choose LR for its popularity in credit scoring, NN for being the best individual classifier and RF for being the best homogeneous ensemble, 




% Our algorithms are compared against NN, LR and RF, which are not strategy-proof. \hl{Prove with  toy counterexample earlier?} We will demonstrate that, while these approaches are known to perform well when the agents are truthful, they can be out-performed by our strategy-proof greedy classifier in the presence of strategic behavior.

\subsection{Results} 
For the sake of exposition, we report results only for $\epsilon = 0.2$. We also limit our exposition of {\sc HC}, {\sc Imp} and {\sc R-F} methods to those based on logistic regression, as these perform better than their {\sc ANN/RF/kNN} counterparts. For a comprehensive compilation of all results, along with standard deviation numbers, please refer to the Supplement.

\paragraph{With a small number of features (Table \ref{tab:accuracy,_2_bal,AAAI,FS}):} As expected, the out-of-the-box baselines perform well under truthful reporting, but not with strategic reporting. Our methods are robust to strategic withholding, and in line with the earlier discussion on the potential issues faced by {\sc Mincut} and IC-LR (in Sections \ref{sec:mincut} and \ref{sec:iclr}), we see that
\begin{enumerate*}[label = \textbf{(\alph*)}]
    \item {\sc HC(LR)} performs most consistently, and
    \item in some cases, {\sc Mincut} (e.g., Poland) and {\sc IC-LR} (e.g., Taiwan) do not do well.
\end{enumerate*}

\begin{table}
\centering
\caption{Our methods vs. the rest: mean classifier accuracy for $\epsilon=0.2$, balanced datasets, 4 features }%("w/ disc." stands for "with discretization of features", "Tru." for "truthful reporting", and "Str." for "strategic reporting").}
\fontsize{9pt}{9pt}\selectfont
\setlength{\tabcolsep}{4.3pt}
\begin{tabular}{@{}lcccccccc@{}}\toprule
\multirow{2}{*}[-3pt]{\makecell[l]{Classifier}} & \multicolumn{2}{c}{Australia} &  \multicolumn{2}{c}{Germany} &  \multicolumn{2}{c}{Poland} &  \multicolumn{2}{c}{Taiwan}\\
\cmidrule(l{5pt}r{5pt}){2-3} \cmidrule(l{5pt}r{5pt}){4-5} \cmidrule(l{5pt}r{5pt}){6-7} \cmidrule(l{5pt}r{5pt}){8-9}
& \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.} & \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.} & \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.} & \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.}\\ \midrule
{\sc HC(LR)} & .792  & {\bf.792} & .639  & .639 & .659  & .659 & .648 & .648\\
%HC (ANN) & .775  & .775 & .624  & .624 & .640  & .640 & .647 & .647\\
{\sc Mincut} & .770  & .770 & .580  & .580 & .501  & .501 & .652 & {\bf .652}\\

{\sc IC-LR} & .788  & .788 & .654  & {\bf .654} & .639  & .639 & .499 & .499\\
%IC-LR w/ neg. & .794  & .794 & {\bf .664}  & {\bf .664} & .646  & .646 & .669 & {\bf .669}\\
\hdashline
%{\sc Maj} & .664  & .674 & .537  & .526 & .501  & .501 & .678 & .560\\

{\sc Imp(LR)} & .796  & .791 & {\bf .663}  & .580 & .{\bf 714}  & {\bf.660} & {\bf .670} & .618\\
%ANN (Imp) & .799  & .789 & {\bf .664}  & .582 & .704  & .643 & {\bf.686} & .536\\
%RF (Imp) & .771  & .630 & .623  & .560 & {\bf .721}  & .602 & .679 & .548\\
%kNN (Imp) & .789  & .721 & .636  & .568 & .695  & .623 & .659 & .559\\

{\sc R-F(LR)} & {\bf .808}  & .545 & .631  & .508 & .670  & .511 & .665 & .590\\
%ANN (R-F) & .804  & .543 & .628  & .509 & .664  & .509 & .668 & .548\\
%RF (R-F) & .777  & .538 & .608  & .508 & .699  & .519 & .679 & .574\\
%kNN (R-F) & .779  & .534 & .602  & .505 & .657  & .512 & .658 & .585\\
\bottomrule
\end{tabular}
\label{tab:accuracy,_2_bal,AAAI,FS}
\end{table}

\paragraph{With discretization (Table \ref{tab:accuracy,_2_bal,AAAI,FS,disc}):} As expected, discretization of numerical features into binary categories improves the performance of {\sc Mincut} and {\sc IC-LR}, for reasons explained in Sections \ref{sec:mincut} and \ref{sec:iclr} respectively. We also see some benefit from discretization for {\sc HC(LR)} when the features are mostly continuous (e.g., Poland), and less so when they are already discrete (e.g., Taiwan).



\begin{table}
\centering
\caption{Our methods vs. the rest: mean classifier accuracy for $\epsilon=0.2$, balanced datasets, 4 features (``w/ disc." stands for ``with discretization of features")}%, "Tru." for "truthful reporting", and "Str." for "strategic reporting").}
\fontsize{9pt}{9pt}\selectfont
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{@{}lcccccccc@{}}\toprule
\multirow{2}{*}[-3pt]{\makecell[l]{Classifier}} & \multicolumn{2}{c}{Australia} &  \multicolumn{2}{c}{Germany} &  \multicolumn{2}{c}{Poland} &  \multicolumn{2}{c}{Taiwan}\\
\cmidrule(l{7pt}r{7pt}){2-3} \cmidrule(l{7pt}r{7pt}){4-5} \cmidrule(l{7pt}r{7pt}){6-7} \cmidrule(l{7pt}r{7pt}){8-9}
& \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.} & \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.} & \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.} & \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.}\\ \midrule
{\sc HC(LR)} w/ disc. & .794  & .794 & .641  & .641 & .692  & .692 & .650 & {\bf.650}\\
%HC (ANN) w/ disc. & .770  & .770 & .614  & .614 & .680  & .680 & .648 & .648\\
{\sc Mincut} w/ disc. & .789  & .789 & .629  & .629 & .692  & .692 & .649 & .649\\

{\sc IC-LR} w/ disc. & {\bf.800}  & {\bf .800} & .651  & {\bf.651} & .698  & {\bf .698} & .646 & .646\\\hdashline
%{\sc Maj} w/ disc. & .795  & .627 & .603  & .531 & .714  & .564 & .688 & .566\\

{\sc Imp(LR)} w/ disc. & .799  & .762 & {\bf.652}  & .577 & {\bf.719}  & .631 & {\bf .686} & .541\\
%ANN (Imp) w/ disc. & .799  & .747 & .652  & .577 & .718  & .635 & .688 & .542\\
%RF (Imp) w/ disc. & .796  & .744 & .643  & .575 & .715  & .620 & {\bf .689} & .542\\
%kNN (Imp) w/ disc. & .786  & .704 & .628  & .572 & .696  & .606 & .655 & .563\\

{\sc R-F(LR)} w/ disc. & .796  & .542 & .633  & .516 & .708  & .522 & .684 & .587\\
%ANN (R-F) w/ disc. & .792  & .544 & .629  & .514 & .707  & .521 & .684 & .541\\
%RF (R-F) w/ disc. & .799  & .546 & .625  & .515 & .706  & .525 & .687 & .585\\
%kNN (R-F) w/ disc. & .775  & .538 & .618  & .512 & .684  & .519 & .651 & .587\\
\bottomrule
\end{tabular}
\label{tab:accuracy,_2_bal,AAAI,FS,disc}
\end{table}

\paragraph{With a large number of features (Table \ref{tab:accuracy,_2_bal,AAAI,NFS}):} 
We see broadly similar trends here, except that in the case with discretization, {\sc IC-LR} performs much better than before (e.g., Poland). The reason for this is that {\sc IC-LR} is able to use all the available features once they are discretized into binary categories. However, without discretization, {\sc HC} methods are more reliable (e.g., Poland and Taiwan).

\begin{table}
\centering
\caption{Our methods vs. the rest: mean classifier accuracy for $\epsilon=0.2$, balanced datasets, all features }%("w/ disc." stands for "with discretization of features", "Tru." for "truthful reporting", and "Str." for "strategic reporting").}
\fontsize{9pt}{9pt}\selectfont
\setlength{\tabcolsep}{1.9pt}
\begin{tabular}{@{}lcccccccc@{}}\toprule
\multirow{2}{*}[-3pt]{\makecell[l]{Classifier}} & \multicolumn{2}{c}{Australia} &  \multicolumn{2}{c}{Germany} &  \multicolumn{2}{c}{Poland} &  \multicolumn{2}{c}{Taiwan}\\
\cmidrule(l{7pt}r{7pt}){2-3} \cmidrule(l{7pt}r{7pt}){4-5} \cmidrule(l{7pt}r{7pt}){6-7} \cmidrule(l{7pt}r{7pt}){8-9}
& \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.} & \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.} & \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.} & \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.}\\ \midrule
{\sc HCfs(LR)}& .795  & .795 & .625  & .625 & .678  & .678 & .648 & .648\\
{\sc HCapp(LR)} & .777  & .777 & .617  & .617 & .658  & .658 & .638 & .638\\
{\sc Mincut} & .496  & .496 & .499  & .499 & .499  & .499 & .499 & .499\\
{\sc IC-LR} & .798  & .798 & .654  & {\bf .654} & .607  & .607 & .588 & .588\\
%IC-LR w/ neg. & .806  & {\bf .806} & .661  & {\bf .661} & .586  & .586 & .662 & .662\\
\hdashline


{\sc HCfs(LR)} w/ disc. & .794  & .794 & .632  & .632 & .694  & .694 & .649 & .649\\
{\sc HCapp(LR)} w/ disc. & .782  & .782 & .620  & .620 & .724  & .724 & .644 & .644\\
{\sc Mincut} w/ disc. & .534  & .534 & .503  & .503 & .499  & .499 & .550 & .550\\
{\sc IC-LR} w/ disc. & .805  & {\bf .805} & .653  & .653 & .773  & {\bf .773} & .667 & {\bf .667}\\\hdashline

{\sc Imp(LR)} & .802  & .701 & {\bf .663}  & .523 & .729  & .507 & .657 &.501 \\ 
{\sc Imp(LR)} w/ disc. & {\bf .809}  & .723 & .659  & .554 & {\bf .783}  & .503 & {\bf .697} & .501\\
\bottomrule
\end{tabular}
\label{tab:accuracy,_2_bal,AAAI,NFS}
\end{table}


\paragraph{On the out-of-the-box baselines:}
\begin{itemize*}
% In \Cref{fig:varyingm}, we present a box plot of the accuracy of various classifiers across our experiments, under strategic reporting. For the sake of exposition, out of all the out-of-box-methods, we include just LR (both Imputation and Reduced Feature variants). In addition to reinforcing the above-mentioned takeaways, Figure \ref{fig:varyingm} leads to a few more interesting observations:
    \item \emph{Imputation-based methods} 
    %perform relatively well compared to other methods in (Figure \ref{fig:varyingm}, Australia), slightly worse in (Figure \ref{fig:varyingm}, Poland), and with high variance in (Figure \ref{fig:varyingm}, Germany). We believe this is because these methods 
    are sensitive vis-\'a-vis the mean/mode values used. There is incentive to drop a certain feature if the imputed value is a positive signal. If there are many such features, then these methods perform poorly, as seen in Table \ref{tab:accuracy,_2_bal,AAAI,NFS} (cf. Table \ref{tab:accuracy,_2_bal,AAAI,FS}, Australia). 
    %if the imputed values are generally a negative signal, then agents have little incentive to withhold features, and these methods perform well (e.g., Australia); if the imputed values are generally a positive signal, then agents would withhold features, and these methods perform worse (e.g., Poland); 
    %for instance, if the imputed value for a feature is a positive signal, then , and hence these methods perform poorly (e.g., Table \ref{tab:accuracy,_2_bal,AAAI,NFS}, Poland). If the imputed values are generally a negative signal, these methods perform well (e.g., Table \ref{tab:accuracy,_2_bal,AAAI,NFS}, Poland)  
    If the imputed values do not give a clear signal (e.g., when the distribution of each feature value is not skewed), there is a high variance in the performance of these methods (see the Supplement). In some cases, the benchmarks perform as well as, or slightly better than, our incentive-compatible classifiers. For example, in Table \ref{tab:accuracy,_2_bal,AAAI,FS}, for the Australia and Poland data sets, the accuracy of {\sc Imp(LR)} and that of {\sc HC(LR)} are within $0.001$ of each other. This happens because the imputed values are, in these cases (but not in most of our other cases), negative indicators of the positive label, and therefore there is generally no incentive to strategically drop features.
    \item \emph{Reduced-Feature modeling}, despite performing well under truthful reporting, allows too many examples to be accepted under strategic reporting, which hurts its performance. This is true especially for smaller $\epsilon$, as each subclassifier has fewer examples to train on, giving several viable options for strategic withholding.
    %\vc{(probably question for Hanrui) is this related to IC generalizing better as in the other paper?}
    %\hz{with all the subclassifiers and stuff involved i feel the connection is quite weak, so probably we shouldn't mention that...  also the main issue here is we are not doing erm in the presence of strategic behavior, which probably introduces far more error than from generalization}
\end{itemize*}

We note here that the variance (in the accuracy achieved) produced by our methods, since they are robust to strategic withholding, is much smaller than that of the baseline methods (exact numbers are deferred to the Supplement).


%We notice the poor performance of {\sc Mincut}: as expected, very few training data points have overlapping feature set, preventing {\sc Mincut} from creating dependencies within the data distribution \hl{better wording?}. HC App. (LR) performs well but is inferior to IC-LR; we suspect it can be improved by more carefully selected subclassifiers. This is a direction for future work. On the other hand, LR (Imp) performs poorer with all features then with 4 features due to having more possible combinations of strategies to be withheld.
% The main takeaways from these numbers are the following:
% \begin{itemize*}  
%     \item At least one of the {\sc HC} and {\sc Mincut} variants outperforms all out-of-the-box classifiers under strategic reporting..
    % \item Discretization helps {\sc HC} and {\sc Mincut} when the features are mostly continuous (e.g., Poland), and naturally, not when the data is already discrete (e.g., Taiwan).
% \end{itemize*}
% And as expected, under truthful reporting, the standard out-of-the-box methods perform better, especially LR (Imputation). However, LR (Imputation, and also, Reduced Feature) do not perform well under strategic reporting (especially in Germany and Taiwan, where the data is more discrete), as we discuss next.

% When 

% In addition to reinforcing the above-mentioned takeaways, Figure \ref{fig:varyingm} leads to a few more interesting observations about why the out-of-the-box classifiers fail: \begin{itemize*}


%Otherwise, increasing the value of $\epsilon$ results in a general downward trend in the accuracy of all classifiers, as there is less information to learn from. 

%Among all the out-of-the-box classifiers, RF is consistently the best under truthful reporting, with (Table \ref{tab:accuracy_with_m=0.2}) or without missing data (Table \ref{tab:allft}), but LR with imputation stands out in the presence of strategic behavior (Str.) when limiting to 4 features (Table \ref{tab:accuracy_with_m=0.2}). 
%\vc{This last part is already about Table \ref{tab:accuracy_with_m=0.2} right? also the tables need more explanation -- what is ``performance,'' not sure everyone will figure out ``Str'' and ``Tru'' ... also I'd put Tru before Str because Tru is the standard case.  Also I think it's common to make the best number in a column bold right?} \hl{Todo: bold font the final tables}. In the case of $\epsilon=0.2$, a good amount of data is naturally missing, yet the classification task is still quite feasible. Here, even when data may be strategically withheld, imputation manages to allow classifiers to achieve an accuracy that is close to what they can achieve in the truthful case on some data sets. 
%Reduced-feature modeling, \hl{despite performing comparably to imputation when behavior is truthful}, allows too many examples to be accepted when strategic behavior is possible, significantly hurting performance.
%accepted, yielding a very high acceptance rate for out-of-the-box classifiers in the presence of strategic behavior. 

%Increasing the value of $\epsilon$ results in a general downward trend in the accuracy of all classifiers, as there is less information to learn from (Figure \ref{fig:varyingm}).
%We also observe that the performance of imputation-based methods is highly sensitive to the classifiers' interaction with the mean/mode value used in imputation: if the mean/mode feature values are generally a negative signal, then the classifier trained on the imputed data is safe from strategic behavior (Figure \ref{fig:varyingm}, Australia); if the mean/mode feature values are generally a positive signal, then the classifier trained on the imputed data is prone to strategic withholding of such features (Figure \ref{fig:varyingm}, Poland); if the mean/mode feature values generally do not give a clear signal, which happens when the distribution of each feature value is not skewed, one can observe a high variance in the performance of the classifier trained on the imputed data (Figure \ref{fig:varyingm}, Germany). {\sc Hill-Climbing} and {\sc Mincut}, on the other hand, perform relatively consistently.



\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}


% \begin{table*}\centering
% \caption{PreFS: Our methods vs. the rest: mean classifier accuracy for $\epsilon=0.2$, balanced datasets ("w/ disc." stands for "with discretization of features", "Tru." for "truthful reporting", and "Str." for "strategic reporting").}
% \small
% \begin{tabular}{@{}lccccccccccc@{}}\toprule
% \multirow{2}{*}[-3pt]{\makecell[l]{Classifier}} & \multicolumn{2}{c}{Australia} & \phantom{}& \multicolumn{2}{c}{Germany} & \phantom{} & \multicolumn{2}{c}{Poland} & \phantom{} & \multicolumn{2}{c}{Taiwan}\\
% \cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12}
% & \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.} && \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.} && \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.} && \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.}\\ \midrule
% HC (LR) & .792 (.022) & .792 (.022) && .639 (.029) & .639 (.029) && .659 (.030) & .659 (.030) && .648 (.006) & .648 (.006)\\
% HC (LR) w/ disc. & .794 (.024) & {\bf .794} (.024) && .641 (.027) & {\bf .641} (.027) && .692 (.026) & {\bf .692} (.026) && .650 (.005) & .650 (.005)\\
% HC (ANN) & .775 (.028) & .775 (.028) && .624 (.029) & .624 (.029) && .640 (.035) & .640 (.035) && .647 (.006) & .647 (.006)\\
% HC (ANN) w/ disc. & .770 (.032) & .770 (.032) && .614 (.035) & .614 (.035) && .680 (.027) & .680 (.027) && .648 (.006) & .648 (.006)\\
% {\sc Mincut} & .770 (.031) & .770 (.031) && .580 (.032) & .580 (.032) && .501 (.017) & .501 (.017) && .652 (.005) & {\bf .652} (.005)\\
% {\sc Mincut} w/ disc. & .789 (.025) & .789 (.025) && .629 (.030) & .629 (.030) && .692 (.026) & {\bf .692} (.026) && .649 (.006) & .649 (.006)\\
% LR-IC (L2) & .787 (.021) & .787 (.021) && {\bf .653} (.027) & {\bf .653} (.027) && .639 (.037) & .639 (.037) && .499 (.004) & .499 (.004)\\
% LR-IC (L2) w/ disc. & {\bf .801} (.020) & {\bf .801} (.020) && .652 (.027) & .652 (.027) && {\bf .696} (.024) & {\bf .696} (.024) && {\bf .646} (.006) & {\bf .646} (.006)\\\hline

% {\sc Maj} & .664 (.025) & .674 (.099) && .537 (.027) & .526 (.043) && .501 (.017) & .501 (.018) && .678 (.005) & .560 (.033)\\
% {\sc Maj} w/ disc. & .795 (.023) & .627 (.095) && .603 (.031) & .531 (.049) && .714 (.024) & .564 (.052) && .688 (.005) & .566 (.034)\\\hdashline

% LR (Imp) & .796 (.021) & .791 (.035) && .663 (.026) & .580 (.081) && .714 (.027) & .660 (.035) && .670 (.008) & .618 (.046)\\
% LR (Imp) w/ disc. & .799 (.021) & .762 (.068) && .652 (.025) & .577 (.083) && .719 (.023) & .631 (.087) && .686 (.006) & .541 (.022)\\
% ANN (Imp) & .799 (.021) & .789 (.038) && {\bf .664} (.025) & .582 (.083) && .704 (.032) & .643 (.044) && .686 (.006) & .536 (.005)\\
% ANN (Imp) w/ disc. & .799 (.021) & .747 (.086) && .652 (.030) & .577 (.084) && .718 (.023) & .635 (.084) && .688 (.005) & .542 (.023)\\
% RF (Imp) & .771 (.023) & .630 (.101) && .623 (.031) & .560 (.065) && {\bf .721} (.021) & .602 (.065) && .679 (.005) & .548 (.031)\\
% RF (Imp) w/ disc. & .796 (.024) & .744 (.089) && .643 (.029) & .575 (.081) && .715 (.024) & .620 (.087) && {\bf .689} (.006) & .542 (.027)\\
% kNN (Imp) & .789 (.023) & .721 (.084) && .636 (.029) & .568 (.069) && .695 (.026) & .623 (.047) && .659 (.020) & .559 (.036)\\
% kNN (Imp) w/ disc. & .786 (.027) & .704 (.120) && .628 (.041) & .572 (.073) && .696 (.048) & .606 (.085) && .655 (.045) & .563 (.050)\\\hdashline

% LR (R-F) & {\bf .808} (.021) & .545 (.063) && .631 (.028) & .508 (.026) && .670 (.030) & .511 (.026) && .665 (.009) & .590 (.038)\\
% LR (R-F) w/ disc. & .796 (.021) & .542 (.068) && .633 (.027) & .516 (.038) && .708 (.022) & .522 (.043) && .684 (.005) & .587 (.029)\\
% ANN (R-F) & .804 (.022) & .543 (.063) && .628 (.028) & .509 (.026) && .664 (.037) & .509 (.026) && .668 (.008) & .548 (.047)\\
% ANN (R-F) w/ disc. & .792 (.021) & .544 (.065) && .629 (.032) & .514 (.036) && .707 (.025) & .521 (.040) && .684 (.006) & .541 (.041)\\
% RF (R-F) & .777 (.024) & .538 (.051) && .608 (.031) & .508 (.025) && .699 (.022) & .519 (.030) && .679 (.005) & .574 (.027)\\
% RF (R-F) w/ disc. & .799 (.022) & .546 (.064) && .625 (.028) & .515 (.036) && .706 (.025) & .525 (.044) && .687 (.005) & .585 (.026)\\
% kNN (R-F) & .779 (.024) & .534 (.055) && .602 (.031) & .505 (.025) && .657 (.028) & .512 (.028) && .658 (.018) & .585 (.029)\\
% kNN (R-F) w/ disc. & .775 (.024) & .538 (.064) && .618 (.032) & .512 (.034) && .684 (.033) & .519 (.037) && .651 (.036) & .587 (.027)\\
% \bottomrule
% \end{tabular}
% \label{tab:accuracy,_2_bal,AAAI_preFS}
% \end{table*}





% \begin{table*}\centering
% \caption{FS: Our methods vs. the rest: mean classifier accuracy for $\epsilon=0.2$, balanced datasets ("w/ disc." stands for "with discretization of features", "Tru." for "truthful reporting", and "Str." for "strategic reporting").}
% \small
% \begin{tabular}{@{}lccccccccccc@{}}\toprule
% \multirow{2}{*}[-3pt]{\makecell[l]{Classifier}} & \multicolumn{2}{c}{Australia} & \phantom{}& \multicolumn{2}{c}{Germany} & \phantom{} & \multicolumn{2}{c}{Poland} & \phantom{} & \multicolumn{2}{c}{Taiwan}\\
% \cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12}
% & \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.} && \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.} && \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.} && \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.}\\ \midrule
% HC (LR) & .795 (.023) & .795 (.023) && .627 (.032) & .627 (.032) && .675 (.033) & .675 (.033) && .648 (.005) & .648 (.005)\\
% HC (LR) w/ disc. & .794 (.021) & .794 (.021) && .635 (.030) & {\bf .635} (.030) && .694 (.032) & .694 (.032) && .650 (.005) & .650 (.005)\\
% HC Approx (LR) & .795 (.018) & .795 (.018) && .635 (.031) & {\bf .635} (.031) && .675 (.034) & .675 (.034) && .648 (.005) & .648 (.005)\\
% HC Approx (LR) w/ disc. & .792 (.020) & .792 (.020) && .633 (.039) & .633 (.039) && .692 (.032) & .692 (.032) && .649 (.005) & .649 (.005)\\
% HC (ANN) & .780 (.027) & .780 (.027) && .618 (.031) & .618 (.031) && .650 (.034) & .650 (.034) && .648 (.005) & .648 (.005)\\
% HC (ANN) w/ disc. & .769 (.027) & .769 (.027) && .609 (.040) & .609 (.040) && .679 (.042) & .679 (.042) && .648 (.006) & .648 (.006)\\
% {\sc Mincut} & .772 (.030) & .772 (.030) && .576 (.033) & .576 (.033) && .498 (.018) & .498 (.018) && .652 (.006) & {\bf .652} (.006)\\
% {\sc Mincut} w/ disc. & .791 (.022) & .791 (.022) && .625 (.029) & .625 (.029) && .693 (.031) & .693 (.031) && .650 (.006) & .650 (.006)\\

% LR-IC (L2) & .790 (.020) & .790 (.020) && .634 (.036) & .634 (.036) && .661 (.041) & .661 (.041) && .498 (.004) & .498 (.004)\\
% LR-IC (L2) w/ disc. & .802 (.020) & {\bf .802} (.020) && .635 (.030) & {\bf .635} (.030) && .695 (.030) & {\bf .695} (.030) && .649 (.006) & .649 (.006)\\\hline
% {\sc Maj} & .666 (.027) & .688 (.082) && .531 (.030) & .539 (.046) && .497 (.017) & .497 (.020) && .679 (.005) & .566 (.031)\\
% {\sc Maj} w/ disc. & .798 (.024) & .628 (.091) && .604 (.040) & .540 (.043) && .707 (.029) & .578 (.057) && .689 (.005) & .568 (.033)\\\hdashline

% LR (Imp) & .798 (.020) & .793 (.028) && {\bf .647} (.027) & .571 (.073) && .709 (.028) & .659 (.046) && .668 (.007) & .620 (.056)\\
% LR (Imp) w/ disc. & .801 (.019) & .761 (.057) && .636 (.028) & .571 (.075) && {\bf .719} (.026) & .552 (.084) && .687 (.005) & .505 (.024)\\
% ANN (Imp) & .801 (.020) & .789 (.036) && {\bf .647} (.027) & .567 (.073) && .709 (.027) & .656 (.044) && .686 (.005) & .535 (.005)\\
% ANN (Imp) w/ disc. & .801 (.017) & .760 (.057) && .636 (.031) & .571 (.072) && .714 (.028) & .566 (.079) && {\bf .690} (.006) & .538 (.018)\\
% RF (Imp) & .771 (.028) & .654 (.093) && .614 (.030) & .544 (.056) && .708 (.028) & .599 (.063) && .680 (.005) & .548 (.030)\\
% RF (Imp) w/ disc. & .796 (.018) & .751 (.079) && .630 (.031) & .569 (.073) && .717 (.026) & .551 (.075) && {\bf .690} (.005) & .539 (.025)\\
% kNN (Imp) & .788 (.022) & .726 (.078) && .624 (.028) & .560 (.066) && .695 (.027) & .611 (.059) && .662 (.014) & .550 (.030)\\
% kNN (Imp) w/ disc. & .786 (.023) & .705 (.124) && .620 (.036) & .561 (.067) && .697 (.052) & .562 (.086) && .662 (.037) & .557 (.044)\\\hdashline

% LR (R-F) & {\bf .807} (.021) & .541 (.053) && .622 (.033) & .508 (.020) && .677 (.026) & .513 (.023) && .666 (.008) & .589 (.044)\\
% LR (R-F) w/ disc. & .798 (.023) & .531 (.044) && .622 (.035) & .520 (.040) && .705 (.029) & .515 (.029) && .686 (.006) & .585 (.033)\\
% ANN (R-F) & .805 (.021) & .538 (.047) && .618 (.031) & .507 (.020) && .674 (.029) & .514 (.021) && .668 (.008) & .541 (.046)\\
% ANN (R-F) w/ disc. & .794 (.024) & .542 (.054) && .617 (.038) & .519 (.042) && .704 (.029) & .522 (.036) && .685 (.006) & .548 (.042)\\
% RF (R-F) & .773 (.025) & .533 (.039) && .600 (.032) & .507 (.021) && .687 (.027) & .522 (.028) && .679 (.005) & .576 (.027)\\
% RF (R-F) w/ disc. & .802 (.022) & .552 (.064) && .616 (.034) & .517 (.035) && .705 (.028) & .524 (.039) && .688 (.005) & .584 (.026)\\
% kNN (R-F) & .778 (.020) & .533 (.048) && .596 (.033) & .504 (.022) && .665 (.026) & .511 (.023) && .663 (.015) & .579 (.030)\\
% kNN (R-F) w/ disc. & .775 (.028) & .533 (.057) && .614 (.038) & .516 (.036) && .681 (.035) & .513 (.020) && .664 (.027) & .588 (.027)\\
% \bottomrule
% \end{tabular}
% \label{tab:accuracy,_2_bal,AAAI_FS}
% \end{table*}





% \begin{table*}
% \centering
% \caption{Our methods vs. the rest: mean classifier accuracy for $\epsilon=0.2$ ("w/ disc." stands for "with discretization of features", "Tru." for "truthful reporting", and "Str." for "strategic reporting"). }
% \small
% \begin{tabular}{@{}lccccccccccc@{}}\toprule
% \multirow{2}{*}[-3pt]{\makecell[l]{Classifier}} & \multicolumn{2}{c}{Australia} & \phantom{}& \multicolumn{2}{c}{Germany} & \phantom{} & \multicolumn{2}{c}{Poland} & \phantom{} & \multicolumn{2}{c}{Taiwan}\\
% \cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12}
% & \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.} && \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.} && \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.} && \multicolumn{1}{c}{Tru.} & \multicolumn{1}{c}{Str.}\\ \midrule
% {\sc HC} (LR) & .793 & .793 && .640 & .640 && .659 & .659 && .648 & .648\\
% {\sc HC} (LR) w/ disc. & .794 & {\bf .794} && .642 & {\bf .642} && .690 & .690 && .650 & .650\\
% {\sc HC} (ANN) & .774 & .774 && .625 & .625 && .640 & .640 && .647 & .647\\
% {\sc HC} (ANN) w/ disc. & .769 & .769 && .617 & .617 && .679 & .679 && .648 & .648\\
% {\sc Mincut} & .768 & .768 && .581 & .581 && .500 & .500 && .652 & {\bf .652}\\
% {\sc Mincut} w/ disc. & .789 & .789 && .630 & .630 && .693 & {\bf .693} && .649 & .649\\ \hline
% {\sc Maj} & .665 & .670 && .539 & .524 && .500 & .500 && .678 & .560\\
% {\sc Maj} w/ disc. & .795 & .618 && .605 & .533 && .715 & .565 && {\bf .688} & .566\\ \hdashline
% LR (Imputation) & .796 & .788 && {\bf .665} & .579 && .715 & .662 && .670 & .619\\
% ANN (Imputation) & .798 & .786 && .665 & .581 && .704 & .648 && .686 & .535\\
% RF (Imputation) & .771 & .630 && .626 & .561 && {\bf .722} & .603 && .679 & .549\\
% kNN (Imputation) & .791 & .722 && .638 & .566 && .694 & .626 && .662 & .560\\ \hdashline
% LR (Reduced Feature) & {\bf.809} & .544 && .632 & .508 && .669 & .510 && .666 & .592\\
% ANN (Reduced Feature) & .806 & .542 && .629 & .509 && .661 & .509 && .668 & .546\\
% RF (Reduced Feature) & .779 & .537 && .611 & .507 && .698 & .518 && .679 & .574\\
% kNN (Reduced Feature) & .781 & .531 && .604 & .505 && .655 & .510 && .658 & .586\\
% \bottomrule
% \end{tabular}
% \label{tab:accuracy_with_m=0.2}
% \end{table*}

\input{conclusion}

\begin{comment}

\newpage
{\sc Beyond Page Limit}

    \begin{figure}[ht]
   \caption{Box plot of classifier accuracy with all features: under strategic reporting}
   \includegraphics[width=0.475\textwidth]{main_NFS_vert.png}
  \label{fig:varyingm}
\end{figure}
\begin{figure}
   \caption{Box plot of classifier accuracy with 4 features: under strategic reporting}
   \includegraphics[width=0.475\textwidth]{main_FS_vert.png}
  \label{fig:varyingm}
\end{figure}





    \begin{figure}
   \caption{Box plot of classifier accuracy with 4 features: under strategic reporting}
   \includegraphics[width=0.475\textwidth]{0601_4box_pcc_bal_fixed.png}
  \label{fig:varyingm}
\end{figure}

\begin{figure}
  \caption{Box plot of classifier accuracy with all features: under strategic reporting}
  \includegraphics[width=\textwidth]{0925_4box_pcc_bal_NFS.png}
  \label{fig:varyingm}
\end{figure}

\newpage

\end{comment}
% \paragraph{A note on feature selection} Given that we filter our data sets to just the top $4$ features, we check the accuracy of the imputation classifiers under truthful reporting using all the features available (\cref{tab:allft}). We restrict ourselves to imputation methods here, since they are computationally tractable with a large number of features. When we do this for $\epsilon=0,0.2$, we find that the accuracy achieved is similar to when we use just the top $4$ features (Tables \ref{tab:accuracy_with_m=0.2}, \ref{tab:allft}). Therefore, if we were somehow able to simulate strategic reporting on a large number of features (which is needed to test out-of-the-box methods), it is plausible that our methods working on just the $4$ features will still do better. 

% \begin{table*}\centering
% % \ra{1.3}
% \caption{Mean accuracy without feature selection: imputation methods under truthful reporting }
% \small
% \begin{tabular}{@{}lccccccccccc@{}}\toprule
% \multirow{2}{*}[-3pt]{\makecell[l]{Classifier}} & \multicolumn{2}{c}{Australia} & \phantom{}& \multicolumn{2}{c}{Germany} &
% \phantom{} & \multicolumn{2}{c}{Poland} &
% \phantom{} & \multicolumn{2}{c}{Taiwan}\\
% \cmidrule{2-3} \cmidrule{5-6} \cmidrule{8-9} \cmidrule{11-12}
% & \multicolumn{1}{c}{$\epsilon=0$} & \multicolumn{1}{c}{$\epsilon=.2$} && \multicolumn{1}{c}{$\epsilon=0$} & \multicolumn{1}{c}{$\epsilon=.2$} && \multicolumn{1}{c}{$\epsilon=0$} & \multicolumn{1}{c}{$\epsilon=.2$} && \multicolumn{1}{c}{$\epsilon=0$} & \multicolumn{1}{c}{$\epsilon=.2$}\\ \midrule
% LR (Imp.) & .848 & .803 && .690 & .660 && .746 & .733 && .670 & .657\\
% ANN (Imp.) & .843 & .802 && .685 & .654 && .753 & .740 && .703 & .690\\
% RF (Imp.) & .869 & .822 && .702 & .664 && .812 & .786 && .704 & .696\\
% kNN (Imp.) & .811 & .772 && .655 & .621 && .743 & .720 && .667 & .650\\
% \bottomrule
% \end{tabular}
% \label{tab:allft}
% \end{table*}



==> strategic classification arxiv/greedy.tex <==
\section{Truthful classifiers and {\sc Hill-Climbing}} \label{sec:greedy}
The other drawback of {\sc Mincut}, related to the issue of generalization just discussed, is that it can be hard to interpret meaningfully in a practical setting. In this section, we devise a simpler alternative called {\sc Hill-Climbing}. To help introduce this algorithm, we first present a characterization of truthful classifiers in our setting, since we can limit our focus to them without loss of generality (as discussed in Section~\ref{sec:prelim}). For shorthand, we use the following definition:

\begin{definition}[$F'$-classifier] 
For a subset of features $F' \subseteq F$, a classifier $f$ is said to be an $F'$-classifier if for all $x \in \mathcal{X}$, we have $f(x) = f(x|_{F'})$, and if there exists $i \in F'$ such that $x_i = *$, then $f(x) = 0$.
\end{definition}
In other words, an $F'$-classifier depends only on the values of the features in $F'$, rejecting any $x$ where any of these is empty. We can collect many such classifiers into an ensemble as follows:

\begin{definition}[{\sc Max} Ensemble]
For a collection of classifiers $\mathcal{C} = \{f_j\}$, its {\sc Max} Ensemble classifier is given by $\textsc{Max}_{\mathcal{C}}(.) \coloneqq \max_j f_j(.)$.
\end{definition}
This is equivalent to getting each agent to pick the most favorable classifier from among those in $\{f_j\}$. Now using the above definitions we have the following characterization of truthful classifiers:

\begin{restatable}{theorem}{characterization}
\label{thm:characterization}
    A classifier $f$ is truthful iff $f(.) = \textsc{Max}_{\mathcal{C}}(.)$ for a collection of classifiers $\mathcal{C} = \{f_j\}$ such that, for some $\{F_j\} \subseteq 2^F$,
    %($F$ is the set of all features), 
    each $f_j$ is an $F_j$-classifier . 
\end{restatable}

Now, for any truthful classifier $f$, we can bound the gap between its population loss $\ell_\mathcal{D}(f)$ and its empirical loss on a set of samples $\widehat{\mathcal{X}}$ denoted by $\ell_{\widehat{\mathcal{X}}}(f) \coloneqq \frac1m \sum_{i \in [m]} |f(x_i) - y_i|$. Before stating a theorem to this end, we define the following entities: Let $\mathcal{H}$ be a base hypothesis space over $\mathcal{X}$, and $n \in \{1, \dots, 2^k\}$ be a parameter. Define $d \coloneqq \dvc(\mathcal{H})$ to be the VC dimension of $\mathcal{H}$. Define $\bar{\mathcal{H}}$ as the set of all classifiers that can be written as the {\sc Max} Ensemble of $n$ classifiers in $\mathcal{H}$. 

\begin{restatable}{theorem}{generalization} \label{thm:generalization}
    Let $\widehat{\mathcal{X}} = \{(x_i, y_i)\}_{i \in [m]}$ be $m$ i.i.d. samples from $\mathcal{D}$. For any $f \in \bar{\mathcal{H}}$, for any $\delta > 0$, with probability at least $1 - \delta$, we have $\ell_\mathcal{D}(f) \le \ell_{\widehat{\mathcal{X}}}(f) + O\left(\sqrt{\frac{dn \cdot \log dn \cdot \log m + \log (1 / \delta)}{m}}\right)$.
\end{restatable}

It is easy to see that for any of the commonly used hypothesis spaces -- say $\mathcal{H}$ consists of linear hypotheses -- if a truthful classifier $f$ is in $\mathcal{H}$, then so are the components of the {\sc Max} Ensemble version of $f$ as in Theorem \ref{thm:characterization}. We have, however, stated Theorem \ref{thm:generalization} in slightly more general terms.
%Theorem~\ref{thm:generalization} provides a way to analyze the population loss of a practical approach for the problem we consider --- see Section~\ref{sec:greedy} for more details.

\paragraph{The {\sc Hill-Climbing} classifier:}
In what follows, we present a hill-climbing approach with provable convergence and generalization guarantees. The {\sc Hill-Climbing} classifier, henceforth referred to as {\sc HC}, is of the same form as given by the characterization of truthful classifiers in Theorem~\ref{thm:characterization}.\footnote{\scriptsize And, therefore, is truthful, and inherits Theorem \ref{thm:generalization}.} Intuitively, the approach works by considering a hierarchy of classifiers, organized by the features involved. For example, consider a setting with $k = 3$ features. We make a choice as to what classifiers we use --- say $f_1$ for input of the form $(x_1, *, *)$, $f_2$ for input of the form $(x_1, x_2, *)$, and $f_3$ for input of the form $(x_1, x_2, x_3)$. Any agent with features $1$ and $2$ (but not $3$), for example, should be able to report both features so as to be classified by $f_2$, or feature $2$ to be classified by $f_1$ instead. So in effect, assuming full knowledge of the classifiers, each agent can check all of the classifiers and choose the most favorable one. Without loss of generality, we assume that when a data point does not have all the features required by a classifier, it is automatically rejected.

\begin{algorithm}
   \caption{{\sc Hill-Climbing} (HC) Classifier}
   \label{alg:greedy}
\begin{algorithmic}
    \STATE {\bfseries Input:} data set $\widehat{\mathcal{X}} = \{(x_i, y_i)\}_{i \in [m]}$, n subsets $F_1, F_2, \ldots, F_n$ of F.
    \STATE Initialize: $t \gets 0$, $\{f_1^0, \ldots, f_n^0\}$.
    \WHILE{$\Delta > 0$}
        \FOR{$i = 1, 2, \ldots, n$}
            \STATE $S_i \gets \{(x, y) \in \widehat{\mathcal{X}}: f_j^t(x|_{F_j}) = 0, \forall j \neq i\}$.
            \STATE $f_i^{t+1} = \argmin_{f \in \mathcal{H}} \sum_{(x, y) \in S_i}  |f(x|_{F_i}) - y|$. \label{line-in-alg:agnostic-oracle}
        \ENDFOR
        \STATE $f^* \gets \textsc{Max}_{\{f^{t+1}_1, \ldots, f^{t+1}_n\}}$; $\ell_t = \ell_{\widehat{\mathcal{X}}}(f^*)$
        \STATE $\Delta \gets \ell_t - \ell_{t-1}$; $t \gets t + 1$
    \ENDWHILE
    
    \STATE {\bfseries Return:} $f^*$.
\end{algorithmic}
\end{algorithm}

In short, {\sc HC} (defined formally in Algorithm \ref{alg:greedy}) works as follows:  first choose a hypothesis space $\mathcal{H}$, in order for Theorem \ref{thm:generalization} to apply. Then select $n$ subsets of $F$ (where $n$ is a parameter), say $F_1, F_2, \ldots, F_n$. For each $F_j$, we learn a $F_j$-classifier, say $f_j$, from among those in $H$. Start by initializing these classifiers to any suitable $\{f^0_1, \ldots, f^0_n\}$. In each iterative step, each of the subclassifiers is updated to minimize the empirical loss on the samples that are rejected by all other classifiers. We next show that such an update procedure always converges. To do so, as far as our theoretical analysis goes, we assume we have black-box access to an agnostic learning oracle (Line \ref{line-in-alg:agnostic-oracle} in Algorithm \ref{alg:greedy}). After convergence, the {\sc HC} classifier is obtained as the {\sc Max} Ensemble of these classifiers. The generalization guarantee of Theorem \ref{thm:generalization} applies directly to the {\sc HC} classifier.

\begin{restatable}{theorem}{convergence} \label{thm:convergence}
  Algorithm \ref{alg:greedy} converges.  
\end{restatable}



\paragraph{Connection with {\sc Mincut}:}
The {\sc HC} formulation given above can be thought of as a less complicated version of {\sc Mincut}: some of the edge constraints are ignored with respect to learning the individual classifiers, and are instead factored in via the {\sc Max} function. Say $F_1 \subset F_2$. For some $x$, it is possible that $f_1(x|_{F_1}) = 1$ and $f_2(x|_{F_1}) = 0$. In other words, the individual classifiers could violate the {\sc Mincut} constraints, in order to learn classification functions that generalize well individually, and also collectively thanks to the combined {\sc HC} training procedure.

\paragraph{Implementing {\sc HC}:}
In practice, the classifiers $\{f_1, f_2, \ldots, f_n\}$ in {\sc HC} can be populated with any standard out-of-the-box methods such as logistic regression or neural networks, the choice of which can influence the performance of $f$. In Section 6, we test {\sc HC} with a few such options. The assumption of having access to an agnostic learning oracle does not play a crucial role in practice, with standard training methods performing well enough to ensure convergence.  
%-- we perform feature selection on datasets with a large number of features, and use all possible subsets of the selected features (see Section \ref{sec:experiments}).
Also, {\sc HC} will converge in at most m (number of training examples) iterations, because in each iteration the number of correctly classified examples increases by at least one. (An iteration may need to train n individual classifiers.) This also means there is no difference between checking whether $\Delta > 0$ or $\Delta \ge 1/m$. In our experiments, we run {\sc HC} using $\Delta \ge 10^{-4}$, and convergence is achieved pretty quickly (see the Supplement for exact details).

\paragraph{Choosing subsets:} Note that we are free to choose any  $F_1, F_2, \ldots, F_n$ to define {\sc HC}. Its generalization (via Theorem \ref{thm:generalization}), will depend on the choice of $n$.
As more and more subsets of features are included (and further binning them based on their values), {\sc HC} starts behaving more and more like {\sc Mincut}. In addition, using a large number of subsets increases the computational complexity of {\sc HC}. In practice, therefore, the number of subsets must be limited somehow -- we find that some simple strategies like the following work reasonably well: 
\begin{enumerate*}[label=(\alph*)]
    \item selecting a few valuable features and taking all subsets of those features,
    \item taking all subsets of size smaller than a fixed number $k$, say $k=2$.
\end{enumerate*}
In many practical situations, a few features (possibly putting their values in just a few bins) are often enough to get close to optimal accuracy, also improving interpretability (e.g., see \citet{wang2015falling} or \citet{jung2017simple})
The question of devising a more nuanced algorithm for selecting these subsets merits a separate investigation, and we leave this to future work.






==> strategic classification arxiv/iclr.tex <==
\section{Incentive-Compatible Logistic Regression}\label{sec:iclr}

As we just mentioned, it is challenging to directly apply {\sc HC} and {\sc Mincut} to a large number of features. As we will see, we can address this challenge in various ways to still get very strong performance with {\sc HC}. Moreover, HC enjoys remarkable generality, generalization and convergence guarantees. Nevertheless, we would like to have an algorithm that tries to make use of all the available features, while still being truthful. In this section, we present such an approach, which, as we show later in Section~\ref{sec:experiments}, indeed performs comparably to -- and in some cases better than -- {\sc Mincut} and {\sc HC}. 

Below we present a simple and truthful learning algorithm, Incentive-Compatible Logistic Regression ({\sc IC-LR}), which is a truthful variant of classical gradient-based algorithms for logistic regression.
Recall that in logistic regression, the goal is to learn a set of coefficients $\{\beta_i\}$, one for each feature $i \in F$, as well as an intercept $\beta_0$, such that for each data point $(x, y)$, the predicted label $\hat{y}$ given by
\[
    \hat{y} = \mathbbm{1} \left[ \sigma(\beta_0 + \sum_{i \in F} x_i \cdot \beta_i ) \ge 0.5 \right]
\]
fits $y$ as well as possible, where $\sigma(t) = 1 / (1 + e^{-t})$ is the logistic function.
Roughly speaking, {\sc IC-LR}. (formally defined in Algorithm~\ref{alg:iclr}) works by restricting the coefficients $\{\beta_i\}$ in such a way that dropping a feature (i.e., setting $x_i$ to $0$) can never make the predicted label larger.
If, without loss of generality, all feature values $x_i$ are nonnegative\footnote{\scriptsize If not, they can be suitably translated.}, then this is equivalent to: for each feature $i \in F$, the coefficient $\beta_i \ge 0$.
{\sc IC-LR}. enforces this nonnegativity constraint throughout the training procedure, by requiring a projection step after each gradient step, which projects the coefficients to the feasible nonnegative region by setting any negative coefficient to $0$ (equivalently, an $\ell_1$ projection).


\begin{algorithm}
   \caption{Incentive-Compatible Logistic Regression}
   \label{alg:iclr}
\begin{algorithmic}
    \STATE {\bfseries Input:} data set $\widehat{\mathcal{X}} = \{(x, y)\}$, learning rate $\{\eta_t\}$, $\delta \ge 0$.
    \STATE Initialize: $t \gets 0$, $\{\beta_0, \beta_1, \dots, \beta_k\}$.
    %\STATE let $\sigma$ be the logistic function: $z \mapsto 1 / (1 + e^{-z})$
    \WHILE{$\Delta > \delta$}
        \STATE $g_i \gets 0$ for all $i \in \{0, 1, \dots, k\}$
        \FOR{$(x, y) \in \widehat{\mathcal{X}}$}
            \STATE $g_0 \gets g_0 + \sigma\left(\beta_0 + \sum_{i \in F} x_i \cdot \beta_i\right) - y$
            \FOR{$i \in F$}
                \STATE $g_i \gets g_i + (\sigma\left(\beta_0 + \sum_{i \in F} x_i \cdot \beta_i\right) - y) \cdot x_i$
            \ENDFOR
        \ENDFOR
        \STATE $\forall i \in \{0, 1, \dots, k\}$, $\beta_i \gets \max\{\beta_i - \eta_t \cdot g_i, 0\}$
        \STATE $f^*(x) \coloneqq \mathbbm{1} \left( \sigma\left(\beta_0 + \sum_{i \in F} \beta_i \cdot x_i\right) \ge 0.5 \right)$
        \STATE $\ell_t = \ell_{\widehat{\mathcal{X}}}(f^*)$; $\Delta \gets \ell_t - \ell_{t-1}$; $t \gets t + 1$
    \ENDWHILE
    
    \STATE {\bfseries Return:} $f^*$.
\end{algorithmic}
\end{algorithm}

One potential issue with {\sc IC-LR}. is the following: if a certain feature $x_i \ge 0$ is negatively correlated with the positive classification label, then {\sc IC-LR} is forced to ignore it (since it is constrained to use positive coefficients). To make good use of this feature, we can include an inverted copy $x'_i  = \lambda - x_i$ (where $\lambda$ is chosen such that $x'_i \ge 0$). We could also choose an apt discretization of such features (using cross-validation) and translate the discretized bins into separate binary variables. Such a discretization can account for more complex forms of correlation, e.g., a certain feature's being too high or too low me makes the positive label likelier. In practice, we find that the latter method does better. If such transformations are undesirable, perhaps for reasons of complexity or interpretability, {\sc HC} methods are a safer bet.

%One potential issue with {\sc IC-LR}. is that if all the features are, on average, negatively correlated with the positive classification label, then it cannot learn anything (because it is constrained to use positive coefficients). To make good use of {\sc IC-LR}., we would need to choose an apt discretization of said features (using cross-validation) and translate the discretized bins into separate binary variables. In this way {\sc IC-LR}. can learn a separate dependence on each of the binary variables. In settings where such a discretization is inappropriate, {\sc HC} methods are a safer bet.
%\anilesh{"We notice that {\sc IC-LR}. performs poorly on Taiwan dataset. This is due to that all four features have negative coefficients, which are then projected to 0, resulting in a LR classifier with 0 coefficients.  \hl{This suggests that {\sc IC-LR}. can be improved by breaking up such negative-coefficient numerical features to categorical features that enables the assignment of positive coefficient to categories that correspond to having low numerical value}" can go to the iclr section}. \hl{(Agree. Can you move it?)}

==> strategic classification arxiv/intro.tex <==
\section{Introduction}
Applicants to most colleges in the US are required to submit their scores for at least one of the SAT and the ACT. Both tests are more or less equally popular, with close to two million taking each in 2016 \citep{adams2017race}. Applicants usually take one of these two tests -- whichever works to their advantage.\footnote{\scriptsize\url{https://www.princetonreview.com/college/sat-act}} However, given the growing competitiveness of college admissions, many applicants now take both tests and then strategically decide whether to drop one of the scores (if they think it will hurt their application) or report both.\footnote{\scriptsize\url{https://blog.collegevine.com/should-you-submit-your-sat-act-scores/}} The key issue here is that
%given the natural variation in the choice of tests (i.e., some take both while others take one), 
it is impossible to distinguish between an applicant who takes both tests but reports only one, and an applicant that takes only one test---for example because the applicant simply took the one required by her school,
the dates for the other test did not work with her schedule, or for other reasons that are not strategic in nature.\footnote{\scriptsize\url{https://blog.prepscholar.com/do-you-need-to-take-both-the-act-and-sat}}


Say a college wants to take a principled machine learning approach to making admission decisions based on the scores from these two tests.  For simplicity, assume no other information is available. Assume that the college has enough historical examples that contain the scores of individuals (on whichever tests are taken, truthfully reported) along with the corresponding ideal (binary) admission decisions.\footnote{\scriptsize We make these assumptions more generally throughout the paper.} Based on this data, the college has to choose a decision function that determines which future applicants are accepted. If this function is known to the applicants, they are bound to strategize and use their knowledge of the decision function to decide the scores they report.\footnotemark[\value{footnote}] 
How can the classifier be trained to handle strategic reporting of scores at prediction time?


To see the intricacies of this problem, let us consider a simple example.
\begin{example}
Say the scores for each of the two tests (SAT and ACT) take one of two values: $h$ (for high) or $l$ (for low). Let $*$ denote a missing value. Then there are eight possible inputs (excluding $(*,*)$ since at least one score is required): $(h,h)$, $(h,l)$, $(l,h)$, $(l,l)$, $(h,*)$, $(*,h)$, $(l,*)$ and $(*,l)$. Assume the natural distribution (without any withholding) over these inputs is known, and so are the conditional probabilities of the label $Y \in \{0,1\}$, as shown below:

\begin{table}[ht]
\centering
\small
\caption{True distribution of inputs and targets:} % $*$ denotes a missing value.}
\setlength\tabcolsep{1.75pt}
\begin{tabular}{c|cccccccc}
 $X$ & $(h,h)$ & $(h,l)$& $(l,h)$& $(l,l)$& $(h,*)$& $(*,h)$& $(l,*)$ & $(*,l)$\\ 
 $Pr(X)$ & $1/8$&  $1/8$&  $1/8$&  $1/8$&  $1/8$&  $1/8$&  $1/8$&  $1/8$\\\hline
 $Pr(Y=1 \mid X)$ & $0.9$&  $0.7$&  $0.3$&  $0.1$&  $0.6$&  $0.6$&  $0.2$&  $0.2$\\
 $Pr(Y=0 \mid X)$ & $0.1$&  $0.3$&  $0.7$&  $0.9$&  $0.4$&  $0.4$&  $0.8$&  $0.8$
 \smallskip
\end{tabular}
\label{tab:example1}
\end{table}

Assume $Y=1$ is the more desirable "accept" decision. Then, ideally, we would like to predict $\widehat{Y}=1$ whenever $X \in \{(h,h),(h,l),(h,*),(*,h)\}$. However, the strategic reporting of scores at prediction time effectively means, for example, that an input $(*,h)$ cannot be assigned the accept decision of $\widehat{Y}=1$ unless the same is done for $(l,h)$ as well; otherwise, someone with $(l,h)$ would simply not report the first test, thereby misreporting $(*,h)$ and being accepted. Taking this into account, %a simple calculation here reveals that 
the classifier with minimum error is given by $\widehat{Y}=1$ whenever $X \in \{(h,h),(h,l),(h,*)\}$.
\end{example}

There are many other settings where a similar problem arises. Many law schools now allow applicants to choose between the GRE and the traditional LSAT.\footnote{\scriptsize \url{https://www.ets.org/gre/revised_general/about/law/}}  Recently, as a result of the COVID-19 pandemic, universities have implemented optional pass/fail policies, where students can choose to take some or all of their courses for pass/fail credit, as opposed to a standard letter grade that influences their GPA.  They are often able to decide the status after already knowing their performance in the course. For credit scoring, some individuals might not report some of their information, especially if it is not mandatory by law \citep{florezlopez2010effects}.

The ability of strategic agents to withhold some of their features at prediction time poses a challenge only when the data used to train the classifier has some naturally missing components to begin with. For if not, the {\em principal} -- e.g., the entity deciding on admissions -- can reject all agents that withhold any of their features, thereby forcing them to reveal all features. 
%Our goal, however, is not to account for the organically missing parts of the data. Rather, 
We focus on how a principal can best train classifiers that are robust even when there is strategic withholding of data by agents.  Our methods produce classifiers that eliminate the incentive for agents to withhold data.
%Our goal can also be put slightly differently as follows: Some data might go missing at prediction time, purely for strategic reasons, if any information about the classifier used by the principal is known to agents. We devise methods that prevent this from occurring by eliminating the incentive for agents to withhold data.

\paragraph{Our contributions}
We now describe the key questions we are facing, and how we answer them. Our model is described formally in \emph{Section \ref{sec:prelim}}. All proofs are in the Supplement.

\emph{If the true input distribution is known, can we compute the optimal classifier? (Section \ref{sec:mincut}}) We answer this question in the affirmative by showing that the problem of computing the optimal classifier (Theorem \ref{thm:mincut}) in this setting reduces to the classical Min-cut problem \citep{cormen2009introduction}. This analysis gives us the {\sc Mincut} classifier, which can be computed on the empirical distribution, estimated using whatever data is available. However, since it can potentially give complex decision boundaries, it might not generalize well. 

\emph{Are there simpler classifiers that are robust to strategic withholding of features? (Section \ref{sec:greedy})} We first characterize the structure of classifiers that are ``truthful", i.e., give no incentive to strategically hide features at prediction time (Theorem \ref{thm:characterization}). Using this characterization, 
%we define the {\sc Greedy} classification algorithm, which produces a hierarchical ensemble of out-of-the-box classifiers. W
we devise a hill-climbing procedure ({\sc HC}) to train 
a hierarchical ensemble of out-of-the-box classifiers
and show that the procedure converges (Theorem \ref{thm:convergence}) as long as we have black-box access to an agnostic learning oracle. We also analytically bound the generalization error of {\sc HC} (Theorem \ref{thm:generalization}). The ensemble of {\sc HC} can be populated with any of the 
commonly used classifiers such as logistic regression, {\sc ANN}s, etc. 

Another truthful classifier we present is a modification of Logistic Regression. This method, called {\sc IC-LR} (Incentive Compatible Logistic Regression), works by encoding all features with positive values, and using positive regression coefficients -- whereby it is in every agent's best interest to report all features truthfully. {\sc IC-LR} uses Projected Gradient Descent for its training. The advantage of this method is that it can be directly to a large number of features.

\emph{How do our methods perform on real data sets? (Section \ref{sec:experiments})} We conduct experiments on several real-world data sets to test the performance of our methods, comparing them to each other, as well as to other methods that handle missing data but ignore the strategic aspect of the problem. We see that our methods perform well overall, and uncover some interesting insights on their relative performance:
\begin{enumerate}%[label=(\alph*)]
    \item When the number of features is small, {\sc HC} is the most reliable across the board.
    \item When the number of features is small, and many of them are discrete/categorical (or suitably discretized), {\sc Mincut} and {\sc IC-LR} perform better.
    \item If a large number of features must be used, {\sc IC-LR} gives the best performance, although {\sc HC} performs reasonably well with some simple feature selection techniques.
\end{enumerate}

\paragraph{Related work}
Our work falls broadly in the area of {\em strategic machine learning}, wherein a common assumption is that strategic agents can modify their features (i.e., misreport) in certain ways (normally at some cost), either to improve outcomes based on the classifier chosen by the principal \citep{hardt2016strategic} or to influence which classifier is chosen in the first place \citep{dekel2010incentive}. The main challenge in strategic machine learning, as in this paper, is the potential misalignment between the interests of the agents and the principal. Existing results in this line of work \citep{chen2018strategyproof,kleinberg2019classifiers,haghtalab2020maximizing}, often mainly theoretical, consider classifiers of a specific form, say linear, and ways of misreporting or modifying features in that context. Our results are different in that we focus on a specific type of strategic misreporting, i.e., withholding parts of the data, and devise general methods that are robust to this behavior that, in addition to having theoretical guarantees, can be tested practically. Some experimental results \citep{hardt2016strategic} do exist -- but our work is quite different; for instance, we do not need to invent a cost function (as in \citet{hardt2016strategic}). Another major difference is that we consider generalization in the presence of strategic behavior, while most previous work does not (except for a concurrent paper \citep{zhang2021incentive}), which studies the sample complexity of PAC learning in the presence of strategic behavior).

Our problem can also be viewed as an instance of {\em automated mechanism design with partial verification} \citep{green1986partially,yu2011mechanism,kephart2015complexity,kephart2016revelation} where it is typically assumed that the feature space (usually called type space in mechanism design) is discrete and has reasonably small cardinality, and a prior distribution is known over the feature space. In contrast, the feature spaces considered in this paper consist of all possible combinations of potentially continuous feature values. Moreover, the population distribution can only be accessed by observing examples. Thus, common methodologies in automated mechanism design do not suffice for our setting.

A set of closely related (in particular, to Theorem \ref{thm:mincut}) theoretical results are those of \citet{zhang2019samples,zhang2019distinguishing,zhang2021classification} on the problem of distinguishing ``good'' agents from ``bad'' %and vice versa 
(where each produces a different distribution over a sample space, and the agent can misreport the set of $n$ samples that she has drawn). However, our work is different in that we consider the standard classification problem, we focus more on practical aspects, and we do not rely on the full knowledge of the input distribution.

Our work also finds a happy intersection between strategic machine learning and the literature on classification with missing data \citep{marlin2008missing}. The problem we study is also connected to \textit{adversarial classification} \citep{dalvi2004adversarial,dekel2010learning}. We discuss these connections in more detail in the Supplement.








==> strategic classification arxiv/mincut.tex <==
\section{The {\sc Mincut} Classifier} \label{sec:mincut}
We first present a method for computing an optimal classifier {\em when the input distribution is fully known}.\footnote{\scriptsize
A theoretical companion paper \cite{zhang2021automated} contains a more general version of the mincut-based algorithm.
There, the goal is to compute an optimal classifier with possibly more than 2 outcomes given perfect knowledge of the entire population distribution.
In this paper, we investigate the special case with only 2 outcomes (i.e., accept and reject), but do not assume prior knowledge about the population distribution.
} Assuming $\mathcal{X}$ is finite, our goal is to characterize a classifier $f^*$ which minimizes the loss $\ell_\mathcal{D}(.)$, for a known input distribution $\mathcal{D}$. As shorthand, define, for all $x \in \mathcal{X}$,
\begin{definition}\label{def:Dplusminus}
    $\mathcal{D}^+(x) \coloneqq \Pr_{(x', y') \sim \mathcal{D}}[x' = x \wedge y' = 1], \\ \quad \mathcal{D}^-(x) \coloneqq \Pr_{(x', y') \sim \mathcal{D}}[x' = x \wedge y' = 0]$.
\end{definition}

The basic idea here is simple: to partition $\mathcal{X}$ into two sides, one labeled $1$ and the other $0$, where the error accrued for each $x \in \mathcal{X}$ is given by $\mathcal{D}^-(x)$ or $\mathcal{D}^+(x)$, according as $x$ is labeled $1$ or $0$. Such a partition should crucially respect the constraints %\footnote{Respecting these constraints makes {\sc Mincut} truthful.} 
imposed by the strategic behavior of agents : if $x \to x'$, then either $x$ is labeled $1$ or $x'$ is labeled $0$.

\begin{definition}\label{def:G_dx}
 Given $\mathcal{X}$ and $\mathcal{D}$, let $G(\mathcal{D}, \mathcal{X})$ be a directed capacitated graph with vertices $V = \mathcal{X} \cup \{s, t\}$, where the edges $E$ and edge capacities $u$ are defined as follows:
    \begin{itemize}
        \item For each $x \in \mathcal{X}$, there are edges $(s, x)$ and $(x,t)$ in $E$, with capacities $u(s, x) = \mathcal{D}^-(x)$ and $u(x, t) = \mathcal{D}^+(x)$.
        \item For all pairs $x, x' \in \mathcal{X}$ such that $x \to x'$, there is an edge $(x, x') \in E$ with capacity $u(x, x') = \infty$.
    \end{itemize}
\end{definition}

\begin{comment}
\begin{definition}\label{def:G_dx}
 Given $\mathcal{X}$ and $\mathcal{D}$, let $G(\mathcal{D}, \mathcal{X})$ be a directed capacitated graph with vertices $V = \mathcal{X} \cup \{s, t\}$, where the edges $E$ and edge capacities $u$ are defined as follows:
    \begin{itemize}
        \item For each $x \in \mathcal{X}$, there is an edge $(s, x) \in E$ with capacity $u(s, x) = \mathcal{D}^-(x)$, and an edge $(x, t) \in E$ with capacity $u(x, t) = \mathcal{D}^+(x)$.
        \item For all pairs $x, x' \in \mathcal{X}$ such that $x \to x'$, there is an edge $(x, x') \in E$ with capacity $u(x', x) = \infty$.
    \end{itemize}
\end{definition}
\end{comment}

In terms of the graph defined above, computing the optimal classifier $f^*$ we seek is equivalent to finding a minimum $s$-$t$ cut on $G(\mathcal{D}, \mathcal{X})$. The intuition is that the edges from $s$ and to $t$ reflect the value gained from labeling an example $0$ or $1$, respectively; one of the edges must be cut, reflecting the loss of not assigning it to the corresponding side.  Moreover, if $x \to x'$, then the corresponding edge with infinite capacity prevents the assigning of $0$ to $x$ and $1$ to $x'$.
\begin{restatable}{theorem}{mincut} \label{thm:mincut}
    If $(S, \bar{S})$ is a minimum $s$-$t$ cut of $G(\mathcal{D}, \mathcal{X})$ (where $S$ is on the same side as $s$), then for the classifier $f^*(x) \coloneqq \mathbbm{1}(x \in \bar{S})$, we have $\ell_\mathcal{D}(f^*) = \min_{f} \ell_\mathcal{D}(f)$.
\end{restatable}


We note that, consequently, the optimal classifier can be computed in $\mathrm{poly}(|\mathcal{X}|)$ time. In practice, it is natural to expect that we do not know $\mathcal{D}$ exactly, but have a finite number of samples from it. A more practical option is to apply Theorem~\ref{thm:mincut} to the empirical distribution induced by the samples observed, and hope for the classifier computed from that to generalize to the true population distribution $\mathcal{D}$. 

\paragraph{Implementing {\sc Mincut}} Given a set $\widehat{\mathcal{X}}$ of $m$ i.i.d.~samples from $\mathcal{D}$, let $\widehat{\mathcal{D}}$ be the corresponding empirical distribution over $\widehat{\mathcal{X}}$, and $\bar{\mathcal{X}} \coloneqq \widehat{\mathcal{X}} \cup \{x': x' \to x, \exists x \in \widehat{\mathcal{X}} \}$. The {\sc Mincut} classifier is then obtained by applying Theorem \ref{thm:mincut} to $G(\widehat{\mathcal{D}},\widehat{\mathcal{X}})$, and extending it to $\bar{\mathcal{X}}$ as and when required. Here, note that {\sc Mincut} runs in time $\mathrm{poly}(m)$ (and not $\mathrm{poly}(|\mathcal{X}|)$), since $G(\widehat{\mathcal{D}},\widehat{\mathcal{X}})$ has $m$ nodes, and checking if a test point is in $\bar{\mathcal{X}}$ takes $\mathrm{poly}(m)$ time.

In light of traditional wisdom, the smaller $m$ is relative to $\mathcal{X}$, the larger the generalization error of {\sc Mincut} will be. We do not attempt a theoretical analysis in this regard, but note that when $\mathcal{X}$ is large, the generalization error can be extremely large (see Example 2 in the Supplement). The reason for this is two-fold: \begin{enumerate}
    \item {\sc Mincut} can give complicated decision boundaries.
    \item {\sc Mincut} is indecisive on samples not in $\bar{\mathcal{X}}$.\footnote{\scriptsize This is more likely to happen when using a large number of features.}
\end{enumerate}
Therefore, a suitable discretization of features is sometimes useful (see Section \ref{sec:experiments}). Note that {\sc Mincut} is truthful, by virtue of the infinite capacity edges in Definition \ref{def:G_dx}.

==> strategic classification arxiv/notes.tex <==
\section{Notes}
\anilesh{
\begin{itemize}
    \item why is the error bar higher for some in Fig 1? Look at a bunch of single runs?
    \item tough to run monotonic with a lot of binary / plain categorical? for each dataset, check which of the categorical variables are ordered, and if there are at least a few, we can try monotonic mincut also.
    \item try AUC for the second fig and see how it looks? \hl{done}
    \item add a few continuous features and see what happens to mincut?
    \item generalization: can we regularize the meta-classifier?
    \item can we do anything with more features where strategic behavior happens?
    \item voting ensembles? \hl{future work}
    \item order of training the classifier within greedy.
    \item majority nearest neighbor
    \item top 4 numerical features -- or different types of features 
    \item why is NN not doing well? Don't claim that they cannot do well ever?
    \item other methods on all features -- otherwise handicapping those methods \hl{cannot test strategic behavior -- too many combinations}
    \item are the lower ones accepting everything
    \item 5/5: 1. N.Neigh non-strategic 2. monotonic
    \item make sure we are not inventing new methods 
    \item still do basic nearest neighbors!
    (KNN)
\end{itemize}}

==> strategic classification arxiv/prelims.tex <==
\section{Preliminaries}
\label{sec:prelim}

We now describe our model and the requisite notation.
\paragraph{Model with strategically withheld features:} We have an input space $\mathcal{X}$, a label space $\mathcal{Y} = \{0, 1\}$, and a distribution $\mathcal{D}$ over $\mathcal{X} \times \mathcal{Y}$ which models the population. A classifier $f: \mathcal{X} \to \mathcal{Y}$ maps a combination of features to a label. Let $F = [k] = \{1, \dots, k\}$ be the set of features, each of which a data point may or may not have.
For $x \in \mathcal{X}$, let $x_i$ denote the value of its $i$-th feature ($x_i = *$ if $x$ does not have feature $i \in [k]$). For any $S \subseteq [k]$, define $x|_S$ to be the projection of $x$ onto $S$ (i.e., retain features in $S$ and drop those not in $S$): 
\begin{align*}
    (x|_S)_i =
    \begin{cases}
        x_i, & \text{if } i \in S \\
        *, & \text{otherwise}.
    \end{cases}
\end{align*}

We assume that data can be strategically manipulated at prediction (test) time in the following way: an agent whose true data point is $x$ can report any other data point $x'$ such that $x|_S = x'$ for some $S \subseteq [k]$. We use $\to$ to denote the relation between any such pair $x, x'$ ($x \to x' \iff \exists S \subseteq [k] : x|_S = x'$). Note that $\to$ is transitive, i.e., for any $x_1, x_2, x_3 \in \mathcal{X}$, $x_1 \to x_2 \text{ and } x_2 \to x_3 \Longrightarrow x_1 \to x_3$. 

We assume agents prefer label $1$ to $0$: in response to a classifier $f$, an agent with data point $x$ will always withhold
\footnote{\scriptsize In practice, $f$ might not be perfectly known, and agents might not be able to best respond. This problem does not arise for our methods, since they are truthul. For other classifiers, their accuracy may go up or down if agents fail to best-respond; but the assumption that agents best-respond is common in many such contexts.} 
features to receive label $1$ if possible, i.e., the agent will report $x' \in \argmax_{x'': x \to x''} f(x'')$. Incorporating such strategic behavior into the loss of a classifier $f$, we get
\begin{align*}
        \ell_\mathcal{D}(f) = \Pr_{(x, y) \sim \mathcal{D}}\left[y \ne \max_{x': x \to x'} f(x') \right].
\end{align*}

\paragraph{Truthful classifiers}
We will also be interested in {\em truthful} classifiers, which provably eliminate incentives for such strategic manipulation. A classifier $f$ is \emph{truthful} if for any $x, x' \in \mathcal{X}$ where $x \to x'$, $f(x) \ge f(x')$.
In other words, not withholding any features is always an optimal way to respond to a truthful classifier.
As a result, the loss of any truthful classifier $f$ in the presence of strategically withheld features has the standard form:
$\ell_\mathcal{D}(f) = \Pr_{(x, y) \sim \mathcal{D}}[f(x) \ne y]$.

Note that the so-called Revelation Principle -- which states that in the presence of strategic behavior, any classifier $f$ is equivalent to a truthful classifier $f'$ -- holds in this case because the reporting structure is transitive.\footnote{\scriptsize More details, including a formal proof, are in the Supplement.}
In other words, we are guaranteed that, for any classifier $f$, there exists a truthful classifier $f'$, such that for any $x \in \mathcal{X}$, $\max_{x': x \to x'} f(x') = f'(x)$. Therefore, we focus on truthful classifiers in our model, without loss of generality.

==> strategic classification arxiv/prelims_old.tex <==
\section{Preliminaries}
\label{sec:prelim}

In this section, we briefly review the PAC learning model under which we will develop our theoretical results, and discuss how strategically dropped features fit in the classical model.

\paragraph{The PAC learning model.}
In the classical PAC learning model, there is a feature space $\mathcal{X}$, a label space $\mathcal{Y} = \{0, 1\}$, and a distribution $\mathcal{D}$ over $\mathcal{X} \times \mathcal{Y}$ which models the population.
A classifier $f: \mathcal{X} \to \mathcal{Y}$ maps a combination of features to a label.
The (population) {\em loss} of a truthful classifier $f$ is defined to be
\[
    \ell_\mathcal{D}(f) = \Pr_{(x, y) \sim \mathcal{D}}[f(x) \ne y].
\]
The smaller the loss is, the better quality the classifier is of.
The goal of PAC learning is to compute a classifier of as small loss as possible, given access to iid labelled samples from the population distribution $\mathcal{D}$.
Note that how small the loss can be generally depends on the number of samples observed.

\paragraph{Strategically dropped features.}
We now extend the PAC learning model to the setting we consider, where features can be strategically dropped.
Let $F = [k] = \{1, \dots, k\}$ be the set of features, each of which a data point may or may not have.
For a data point $x \in \mathcal{X}$, let $x_i$ denote the value of its $i$-th feature.
$x_i = *$ if $x$ does not have feature $i \in [k]$.
For any set of features $S \subseteq [k]$, let $x|_S$ be $x$ projected to $S$, obtained by dropping all features out of $S$.
That is,
\[
    (x|_S)_i =
    \begin{cases}
        x_i, & \text{if } i \in S \\
        *, & \text{otherwise}.
    \end{cases}
\]
A data point with feature values $x$ can report feature values $x'$ (denoted $x \to x'$), iff there exists a set of features $S \subseteq [k]$, such that $x|_S = x'$.
$S = [k]$ corresponds to the case where a data point can always report its complete feature values.
Note that $\to$ is transitive, i.e., for any $x_1, x_2, x_3 \in \mathcal{X}$,
\[
    x_1 \to x_2 \text{ and } x_2 \to x_3 \Longrightarrow x_1 \to x_3.
\]
We assume data points prefer label $1$ to $0$.
In response to a classifier $f$, a data point with feature values $x$ will always drop (or not drop) features in a way such that they receive label $1$ whenever possible, i.e., it will report
\[
    x' \in \argmax_{x'': x \to x''} f(x'').
\]
Such strategic behavior in general affects the loss of the classifier.
Formally, with strategically dropped features, the loss of a classifier $f$ is
\[
    \ell_\mathcal{D}(f) = \Pr_{(x, y) \sim \mathcal{D}}\left[\max_{x': x \to x'} f(x') \ne y\right].
\]

\paragraph{Truthful classifiers.}
Strategically dropped features can be undesirable in various ways.
One may therefore be interested in {\em truthful} classifiers, which provably prevent such strategic manipulation.
A classifier $f$ is truthful, if for any $x, x' \in \mathcal{X}$ where $x \to x'$, $f(x) \ge f(x')$.
In other words, reporting ones complete feature values is always an optimal way to respond to a truthful classifier.
As a result, the loss of any truthful classifier $f$ in the presence of strategically dropped features has the same form of the loss in the classical PAC model, i.e.,
\[
    \ell_\mathcal{D}(f) = \Pr_{(x, y) \sim \mathcal{D}}[f(x) \ne y].
\]
Note that since the reporting structure is transitive, the so-called revelation principal holds (see \cite{zhang2019distinguishing}), which states that any classifier $f$ is equivalent to a truthful classifier $f'$.
Formally, for any classifier $f$, there exists a truthful classifier $f'$, such that for any $x \in \mathcal{X}$,
\[
    \max_{x': x \to x'} f(x') = f'(x).
\]
So without loss of generality, one can focus on truthful classifiers.

==> strategic classification arxiv/references.tex <==
\begin{thebibliography}{40}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Adams(2017)]{adams2017race}
Caralee~J. Adams.
\newblock \emph{In Race for Test-Takers, ACT Outscores SAT—for Now}, 2017.
\newblock URL
  \url{https://www.edweek.org/ew/articles/2017/05/24/in-race-for-test-takers-act-outscores-sat--for.html}.

\bibitem[Amodei et~al.(2016)Amodei, Olah, Steinhardt, Christiano, Schulman, and
  Man{\'e}]{Amodei2016ConcretePI}
Dario Amodei, Chris Olah, Jacob Steinhardt, Paul~F. Christiano, John Schulman,
  and Dan Man{\'e}.
\newblock Concrete problems in ai safety.
\newblock \emph{ArXiv}, abs/1606.06565, 2016.

\bibitem[Chawla et~al.(2003)Chawla, Japkowicz, and Kolcz]{chawla2003icml}
N~Chawla, N~Japkowicz, and A~Kolcz.
\newblock Icml’2003 workshop on learning from imbalanced data sets (ii).
\newblock In \emph{Proceedings available at http://www. site. uottawa.
  ca/nat/Workshop2003/workshop2003. html}, 2003.

\bibitem[Chawla et~al.(2004)Chawla, Japkowicz, and Kotcz]{chawla2004special}
Nitesh~V Chawla, Nathalie Japkowicz, and Aleksander Kotcz.
\newblock Special issue on learning from imbalanced data sets.
\newblock \emph{ACM SIGKDD explorations newsletter}, 6\penalty0 (1):\penalty0
  1--6, 2004.

\bibitem[Chen et~al.(2018)Chen, Podimata, Procaccia, and
  Shah]{chen2018strategyproof}
Yiling Chen, Chara Podimata, Ariel~D Procaccia, and Nisarg Shah.
\newblock Strategyproof linear regression in high dimensions.
\newblock In \emph{Proceedings of the 2018 ACM Conference on Economics and
  Computation}, pages 9--26, 2018.

\bibitem[Conroy et~al.(2016)Conroy, Eshelman, Potes, and
  Xu-Wilson]{conroy2016dynamic}
Bryan Conroy, Larry Eshelman, Cristhian Potes, and Minnan Xu-Wilson.
\newblock A dynamic ensemble approach to robust classification in the presence
  of missing data.
\newblock \emph{Machine Learning}, 102\penalty0 (3):\penalty0 443--463, 2016.

\bibitem[Cormen et~al.(2009)Cormen, Leiserson, Rivest, and
  Stein]{cormen2009introduction}
Thomas~H Cormen, Charles~E Leiserson, Ronald~L Rivest, and Clifford Stein.
\newblock \emph{Introduction to algorithms}.
\newblock MIT press, 2009.

\bibitem[Dalvi et~al.(2004)Dalvi, Domingos, Sanghai, and
  Verma]{dalvi2004adversarial}
Nilesh Dalvi, Pedro Domingos, Sumit Sanghai, and Deepak Verma.
\newblock Adversarial classification.
\newblock In \emph{Proceedings of the tenth ACM SIGKDD international conference
  on Knowledge discovery and data mining}, pages 99--108, 2004.

\bibitem[Daniely et~al.(2015)Daniely, Sabato, Ben-David, and
  Shalev-Shwartz]{daniely2015multiclass}
Amit Daniely, Sivan Sabato, Shai Ben-David, and Shai Shalev-Shwartz.
\newblock Multiclass learnability and the erm principle.
\newblock \emph{The Journal of Machine Learning Research}, 16\penalty0
  (1):\penalty0 2377--2404, 2015.

\bibitem[Dekel et~al.(2010{\natexlab{a}})Dekel, Fischer, and
  Procaccia]{dekel2010incentive}
Ofer Dekel, Felix Fischer, and Ariel~D Procaccia.
\newblock Incentive compatible regression learning.
\newblock \emph{Journal of Computer and System Sciences}, 76\penalty0
  (8):\penalty0 759--777, 2010{\natexlab{a}}.

\bibitem[Dekel et~al.(2010{\natexlab{b}})Dekel, Shamir, and
  Xiao]{dekel2010learning}
Ofer Dekel, Ohad Shamir, and Lin Xiao.
\newblock Learning to classify with missing and corrupted features.
\newblock \emph{Machine learning}, 81\penalty0 (2):\penalty0 149--178,
  2010{\natexlab{b}}.

\bibitem[Dietterich(1998)]{dietterich1998approximate}
Thomas~G Dietterich.
\newblock Approximate statistical tests for comparing supervised classification
  learning algorithms.
\newblock \emph{Neural computation}, 10\penalty0 (7):\penalty0 1895--1923,
  1998.

\bibitem[Dua and Graff(2017)]{Dua:2019}
Dheeru Dua and Casey Graff.
\newblock {UCI} machine learning repository, 2017.
\newblock URL \url{http://archive.ics.uci.edu/ml}.

\bibitem[Elkan(2001)]{elkan2001foundations}
Charles Elkan.
\newblock The foundations of cost-sensitive learning.
\newblock In \emph{International joint conference on artificial intelligence},
  volume~17, pages 973--978. Lawrence Erlbaum Associates Ltd, 2001.

\bibitem[Fayyad and Irani(1993)]{DBLP:conf/ijcai/FayyadI93}
Usama~M. Fayyad and Keki~B. Irani.
\newblock Multi-interval discretization of continuous-valued attributes for
  classification learning.
\newblock In Ruzena Bajcsy, editor, \emph{Proceedings of the 13th International
  Joint Conference on Artificial Intelligence. Chamb{\'{e}}ry, France, August
  28 - September 3, 1993}, pages 1022--1029. Morgan Kaufmann, 1993.
\newblock URL \url{http://ijcai.org/Proceedings/93-2/Papers/022.pdf}.

\bibitem[Florez-Lopez(2010)]{florezlopez2010effects}
Raquel Florez-Lopez.
\newblock Effects of missing data in credit risk scoring. a comparative
  analysis of methods to achieve robustness in the absence of sufficient data.
\newblock \emph{The Journal of the Operational Research Society}, 61\penalty0
  (3):\penalty0 486--501, 2010.

\bibitem[Globerson and Roweis(2006)]{globerson2006nightmare}
Amir Globerson and Sam Roweis.
\newblock Nightmare at test time: robust learning by feature deletion.
\newblock In \emph{Proceedings of the 23rd international conference on Machine
  learning}, pages 353--360, 2006.

\bibitem[Green and Laffont(1986)]{green1986partially}
Jerry~R Green and Jean-Jacques Laffont.
\newblock Partially verifiable information and mechanism design.
\newblock \emph{The Review of Economic Studies}, 53\penalty0 (3):\penalty0
  447--456, 1986.

\bibitem[Haghtalab et~al.(2020)Haghtalab, Immorlica, Lucier, and
  Wang]{haghtalab2020maximizing}
Nika Haghtalab, Nicole Immorlica, Brendan Lucier, and Jack Wang.
\newblock Maximizing welfare with incentive-aware evaluation mechanisms.
\newblock In \emph{29th International Joint Conference on Artificial
  Intelligence}, 2020.

\bibitem[Hand and Anagnostopoulos(2013)]{hand2013area}
David~J Hand and Christoforos Anagnostopoulos.
\newblock When is the area under the receiver operating characteristic curve an
  appropriate measure of classifier performance?
\newblock \emph{Pattern Recognition Letters}, 34\penalty0 (5):\penalty0
  492--495, 2013.

\bibitem[Hardt et~al.(2016)Hardt, Megiddo, Papadimitriou, and
  Wootters]{hardt2016strategic}
Moritz Hardt, Nimrod Megiddo, Christos Papadimitriou, and Mary Wootters.
\newblock Strategic classification.
\newblock In \emph{Proceedings of the 2016 ACM conference on innovations in
  theoretical computer science}, pages 111--122, 2016.

\bibitem[Japkowicz(2000)]{japkowicz2000aaai}
N~Japkowicz.
\newblock Aaai’2000 workshop on learning from imbalanced data sets.
\newblock \emph{AAAI Tech Report, No. WS-00-05}, 2000.

\bibitem[Jung et~al.(2017)Jung, Concannon, Shroff, Goel, and
  Goldstein]{jung2017simple}
Jongbin Jung, Connor Concannon, Ravi Shroff, Sharad Goel, and Daniel~G
  Goldstein.
\newblock Simple rules for complex decisions.
\newblock \emph{Available at SSRN 2919024}, 2017.

\bibitem[Kephart and Conitzer(2015)]{kephart2015complexity}
Andrew Kephart and Vincent Conitzer.
\newblock Complexity of mechanism design with signaling costs.
\newblock In \emph{Proceedings of the 2015 International Conference on
  Autonomous Agents and Multiagent Systems}, pages 357--365, 2015.

\bibitem[Kephart and Conitzer(2016)]{kephart2016revelation}
Andrew Kephart and Vincent Conitzer.
\newblock The revelation principle for mechanism design with reporting costs.
\newblock In \emph{Proceedings of the 2016 ACM Conference on Economics and
  Computation}, pages 85--102, 2016.

\bibitem[Kleinberg and Raghavan(2019)]{kleinberg2019classifiers}
Jon Kleinberg and Manish Raghavan.
\newblock How do classifiers induce agents to invest effort strategically?
\newblock In \emph{Proceedings of the 2019 ACM Conference on Economics and
  Computation}, pages 825--844, 2019.

\bibitem[Lessmann et~al.(2015)Lessmann, Baesens, Seow, and
  Thomas]{lessmann2015benchmarking}
Stefan Lessmann, Bart Baesens, Hsin-Vonn Seow, and Lyn~C Thomas.
\newblock Benchmarking state-of-the-art classification algorithms for credit
  scoring: An update of research.
\newblock \emph{European Journal of Operational Research}, 247\penalty0
  (1):\penalty0 124--136, 2015.

\bibitem[Marlin(2008)]{marlin2008missing}
Benjamin Marlin.
\newblock \emph{Missing data problems in machine learning}.
\newblock PhD thesis, Citeseer, 2008.

\bibitem[Pedregosa et~al.(2011)Pedregosa, Varoquaux, Gramfort, Michel, Thirion,
  Grisel, Blondel, Prettenhofer, Weiss, Dubourg, Vanderplas, Passos,
  Cournapeau, Brucher, Perrot, and Duchesnay]{scikit-learn}
F.~Pedregosa, G.~Varoquaux, A.~Gramfort, V.~Michel, B.~Thirion, O.~Grisel,
  M.~Blondel, P.~Prettenhofer, R.~Weiss, V.~Dubourg, J.~Vanderplas, A.~Passos,
  D.~Cournapeau, M.~Brucher, M.~Perrot, and E.~Duchesnay.
\newblock Scikit-learn: Machine learning in {P}ython.
\newblock \emph{Journal of Machine Learning Research}, 12:\penalty0 2825--2830,
  2011.

\bibitem[Saar-Tsechansky and Provost(2007)]{saar2007handling}
Maytal Saar-Tsechansky and Foster Provost.
\newblock Handling missing values when applying classification models.
\newblock \emph{Journal of machine learning research}, 8\penalty0
  (Jul):\penalty0 1623--1657, 2007.

\bibitem[Shalev-Shwartz and Ben-David(2014)]{shalev2014understanding}
Shai Shalev-Shwartz and Shai Ben-David.
\newblock \emph{Understanding machine learning: From theory to algorithms}.
\newblock Cambridge university press, 2014.

\bibitem[Syed and Taskar(2010)]{syed2010semi}
Umar Syed and Ben Taskar.
\newblock Semi-supervised learning with adversarially missing label
  information.
\newblock In \emph{Advances in Neural Information Processing Systems}, pages
  2244--2252, 2010.

\bibitem[Vorobeychik and Kantarcioglu(2018)]{vorobeychik2018adversarial}
Yevgeniy Vorobeychik and Murat Kantarcioglu.
\newblock Adversarial machine learning.
\newblock \emph{Synthesis Lectures on Artificial Intelligence and Machine
  Learning}, 12\penalty0 (3), 2018.

\bibitem[Wang and Rudin(2015)]{wang2015falling}
Fulton Wang and Cynthia Rudin.
\newblock Falling rule lists.
\newblock In \emph{Artificial Intelligence and Statistics}, pages 1013--1022,
  2015.

\bibitem[Yu(2011)]{yu2011mechanism}
Lan Yu.
\newblock Mechanism design with partial verification and revelation principle.
\newblock \emph{Autonomous Agents and Multi-Agent Systems}, 22\penalty0
  (1):\penalty0 217--223, 2011.

\bibitem[Zhang and Conitzer(2021)]{zhang2021incentive}
Hanrui Zhang and Vincent Conitzer.
\newblock Incentive-aware {PAC} learning.
\newblock In \emph{Proceedings of the AAAI Conference on Artificial
  Intelligence}, 2021.

\bibitem[Zhang et~al.(2019{\natexlab{a}})Zhang, Cheng, and
  Conitzer]{zhang2019distinguishing}
Hanrui Zhang, Yu~Cheng, and Vincent Conitzer.
\newblock Distinguishing distributions when samples are strategically
  transformed.
\newblock In \emph{Advances in Neural Information Processing Systems}, pages
  3187--3195, 2019{\natexlab{a}}.

\bibitem[Zhang et~al.(2019{\natexlab{b}})Zhang, Cheng, and
  Conitzer]{zhang2019samples}
Hanrui Zhang, Yu~Cheng, and Vincent Conitzer.
\newblock When samples are strategically selected.
\newblock In \emph{International Conference on Machine Learning}, pages
  7345--7353, 2019{\natexlab{b}}.

\bibitem[Zhang et~al.(2021{\natexlab{a}})Zhang, Cheng, and
  Conitzer]{zhang2021automated}
Hanrui Zhang, Yu~Cheng, and Vincent Conitzer.
\newblock Automated mechanism design for classification with partial
  verification.
\newblock In \emph{Proceedings of the AAAI Conference on Artificial
  Intelligence}, 2021{\natexlab{a}}.

\bibitem[Zhang et~al.(2021{\natexlab{b}})Zhang, Cheng, and
  Conitzer]{zhang2021classification}
Hanrui Zhang, Yu~Cheng, and Vincent Conitzer.
\newblock Classification with few tests through self-selection.
\newblock In \emph{Proceedings of the AAAI Conference on Artificial
  Intelligence}, 2021{\natexlab{b}}.

\end{thebibliography}


==> strategic classification arxiv/settings.tex <==
%\usepackage{natbib}
\usepackage{makecell}
\usepackage{multicol}
\usepackage{multirow}
\usepackage{amsmath, amssymb, amsthm, amsfonts}
\usepackage{graphicx}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{bbm}
\usepackage{verbatim}
\usepackage{xcolor}
\usepackage{mathtools}

%\usepackage{tabularx}

%\bibliographystyle{plainnat}
\usepackage{bbm}
\usepackage{booktabs}
\usepackage{arydshln}

\usepackage[inline]{enumitem}
\setlist[itemize]{leftmargin=*}
\setlist[enumerate]{leftmargin=*}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{claim}{Claim}
\newtheorem{example}{Example}
\theoremstyle{definition}
\newtheorem{definition}{Definition}

\usepackage{thmtools}
\usepackage{thm-restate}
%\usepackage{hyperref}
\usepackage[capitalise]{cleveref}

%\usepackage{wrapfig}

\usepackage[english]{babel}
\usepackage{blindtext}

\newcommand{\argmax}{\operatorname{argmax}}
\newcommand{\argmin}{\operatorname{argmin}}
\newcommand{\dvc}{d_\mathrm{VC}}

\usepackage{xcolor}
\definecolor{anil}{rgb}{0.8, 0.0, 0.5}
\newcommand{\anilesh}[1]{\textcolor{anil}{ak: #1}}

\newcommand{\david}[1]{{\color{magenta} dr: #1}} 

\newcommand{\hl}[1]{{\color{red} hl: #1}}

\newcommand{\hz}[1]{{\color{cyan} hz: #1}}

\newcommand{\vc}[1]{{\color{blue} vc: #1}}

% \renewcommand{\paragraph}[1]{\textbf{#1}}

